The Benefits of Diligence

This paper studies the strength of embedding Call-by-Name ({\tt dCBN}) and Call-by-Value ({\tt dCBV}) into a unifying framework called the Bang Calculus ({\tt dBANG}). These embeddings enable establishing (static and dynamic) properties of {\tt dCBN} and {\tt dCBV} through their respective counterparts in {\tt dBANG}. While some specific static properties have been already successfully studied in the literature, the dynamic ones are more challenging and have been left unexplored. We accomplish that by using a standard embedding for the (easy) {\tt dCBN} case, while a novel one must be introduced for the (difficult) {\tt dCBV} case. Moreover, a key point of our approach is the identification of {\tt dBANG} diligent reduction sequences, which eases the preservation of dynamic properties from {\tt dBANG} to {\tt dCBN}/{\tt dCBV}. We illustrate our methodology through two concrete applications: confluence/factorization for both {\tt dCBN} and {\tt dCBV} are respectively derived from confluence/factorization for {\tt dBANG}.

==> 4_Factorization_old.tex <==
\newcommand{\nameSectionIV}
    {Factorization}

\section{Factorization}
\label{sec:Factorization}

In $\lambda$-calculi, reduction is a relation, so different reduction
steps are possible starting from the same term. Some steps (\eg head
steps) are more significant than others, and they may occur in the
middle of a \cvictor{reduction}{less significant} sequence.
Factorization is the process of disentangling the significant steps
from the ``superfluous'' ones, bringing the former forward and leaving
the start~and~end~terms~unchanged.

This section is devoted to the factorization property for \BANGSymb,
\CBNSymb and \CBVSymb. We start by revisiting %in \Cref{subsec:Abstract Factorization} 
an abstract factorization theorem~\cite{Accattoli12}.
\cgiulio{Subsequently, i}{I}n \Cref{subsec:Bang Factorization}, we
apply this abstract method to \BANGSymb, thus obtaining a new result
of factorization for the distant Bang calculus not previously
appearing in the literature. To conclude, we use the properties of
simulation and reverse simulation proved in
\Cref{sec:CBN_CBV_Embeddings} to project the factorization result for
\BANGSymb into \CBNSymb (\Cref{subsec:CBN Factorization}) and \CBVSymb
(\Cref{subsec:CBV Factorization}). Although these two results can be
directly derived from the abstract factorization
theorem~\cite{Accattoli12}, our approach circumvents the numerous
commutation properties required by the abstract approach. Also, it
provides a tangible illustration of how the simulation and reverse
simulation properties discussed in
\Cref{subsec:Call-by-Name_Calculus_and_Embedding,subsec:Call-by-Value_Calculus_and_Embedding}
can be applied in~concrete~cases.

\paragraph{Abstract Factorization.}
\label{subsec:Abstract Factorization}

We recall an abstract factorization method from~\cite{Accattoli12}
that relies on local rewrite conditions given by the notion of
\emph{square factorization system} (SFS). While its original
presentation concerns only two subreductions, we (straightforwardly)
extend the notion of SFS to a \emph{family} of
\cvictor{subreducations}{subreductions}, as in our framework with ES
the reduction consists of more than two subreductions.

\begin{definition}
    Let $\mathcal{R} = (R,\, \rightarrow_\rel)$ be an abstract
    rewriting system The family $\left(\arrRExt[\rel_k],
    \arrRInt[\rel_k]\right)_{k \in K}$ of paired reduction relations
    is a \emphasis{square factorization system (SFS)} for
    $\mathcal{R}$ if it covers the reduction relation (\ie
    $\rightarrow_\rel\;= \bigcup_{k \in K} \arrR[\rel_k]$ where
    $\arrR[\rel_k] \,\coloneqq\, \arrRExt[\rel_k] \cup \arrRInt[\rel_k]$) and
    satisfies the following conditions:
    \begin{enumerate}
    \item \textbf{Termination:} %
        $\forall\, k \in K$, $\arrRExt[\rel_k]$ is terminating.

    \item \textbf{Row-swaps:} %
        $\forall\, k \in K$,\; $\arrRInt[\rel_k]\arrRExt[\rel_k]
            \;\subseteq\; \arrpRExt[\rel_{k}]\arrsRInt[\rel_{k}]$.

    \item \textbf{Diagonal-swaps:} %
            $\forall\, k_1, k_2 \in K$, $k_1 \neq k_2$,\;
            $\arrRInt[\rel_{k_1}]\arrRExt[\rel_{k_2}] \;\subseteq\;
            \arrRExt[\rel_{k_2}]\arrsR[\rel_{k_1}]$\!.
        \end{enumerate}%
\end{definition}

The symbol $\circ$ tags \emph{significant} (also called
\emph{external}) steps, while $\bullet$ is used for \emph{\insignificant}
(also called \emph{internal}) ones. 
The commutations required in an
SFS are sufficient to achieve factorization, which consists in
rearranging a reduction sequence to prioritize significant steps
$\arrRExt$ over {\insignificant} steps $\arrRInt$.


\begin{restatable}[\cite{Accattoli12}]{theorem}{RecSFSFactorizable}
    % \LemmaToFromProof{SFS_Factorizable}%
    \label{lem:SFS_Factorizable}%
    Let $\mathcal{R} = (R, \rightarrow_\rel)$ be an abstract rewriting
    system and $(\arrRExt[\rel_k], \arrRInt[\rel_k])_{k \in K}$ be a
    SFS for $\mathcal{R}$. Then the reduction relation factorizes,
    that is, $\rightarrow^*_\rel \ \subseteq \ \rightarrow^*_\circ
    \rightarrow^*_\bullet$ where $\rightarrow_\circ \coloneqq
    \bigcup_{k \in K} \arrRExt[\rel_k]$ and $\rightarrow_\bullet
    \coloneqq \bigcup_{k \in K} \arrRInt[\rel_k]$. 
\end{restatable}
%\begin{proof}
%    Straightforward extension of \cite{Accattoli12}.
%\end{proof}


\subsection{\BANGSymb Factorization}
\label{subsec:Bang Factorization}

In \BANGSymb, we claim that \surface reduction is the
significant part of \full reduction, and our goal is to factor it
out. To exploit the aforementioned abstract method, we first formally identify the \insignificant\ sub-relation of \full
reduction, called here \emph{internal reduction}, as reduction under the scope of a $\oc$. 
\emphasis{Internal contexts}
$\bangICtxt \in \bangICtxtSet$ are full contexts $\bangFCtxtSet$ for
which the hole is placed under a bang. Formally,%
\begin{align*}
	\emphasis{(\BANGSymb Internal Ctxts)}
	& &
	\bangICtxt &\;\Coloneqq\; \oc\bangFCtxt
	\vsep \bangSCtxt^*\bangCtxtPlug{\bangICtxt}
	&&
	\text{with } \bangSCtxt^* \in \bangSCtxtSet \setminus \{\Hole\}
\end{align*}

\noindent
Clearly, $\bangICtxtSet = \bangFCtxtSet \setminus \bangSCtxtSet$.
As usual, $\bangArrSet_I<R>$ is the closure
of the rewrite rules $\rel \in \{\bangSymbBeta, \bangSymbSubs,
\bangSymbBang\}$ over all contexts $\bangICtxt \in \bangICtxtSet$.
The  \emphasis{\BANGSymb internal reduction} is the relation
$\bangArrSet_I \, \coloneqq \, \bangArrSet_I<dB> \cup \bangArrSet_I<s!> \cup \bangArrSet_I<d!>$. For example, $\app[\,]{(\abs{x}{\oc \Hole})}{y} $ is an internal context while $\Hole$ is not. Thus,
$\app[\,]{(\abs{x}{\oc (z\esub{z}{x})})}{y} \bangArrSet_I<s!>
\app[\,]{(\abs{x}{\oc x})}{y} \not\bangArrSet_I (\oc x)\esub{x}{y}$.
%Having this concept at hand, it is now possible to
We can now show that surface
and internal reductions enjoy the abstract properties of an SFS.

\begin{restatable}{lemma}{BangSFS}
    % \LemmaToFromProof{BangSFS}%
    \label{lem:BangSFS}%
    The family  $(\bangArrSet_S<\rel>, \bangArrSet_I<\rel>)_{\rel \in
        \{\bangSymbBeta, \bangSymbSubs, \bangSymbBang\}}$%
    is an SFS for $(\setBangTerms, \bangArr_F)$.
\end{restatable}

This immediately gives the following novel factorization result for
the Distant Bang Calculus, by applying \Cref{lem:SFS_Factorizable} and \Cref{lem:BangSFS}.

\begin{corollary}[\BANGSymb Factorization]
    \label{lem:Bang_Factorization}%
    \quad $\bangArrSet*_F \;=\; \bangArrSet*_S\bangArrSet*_I$.
\end{corollary}

\begin{example} Take $t=(\app{x}{y})\esub{y}{\oc (\app{I}{ \oc
  \oc (\app{I}{ w})})}$ where $I = \abs{z}{z}$. 
Then, the
  factorization of the first sequence starting at $t$ below,
  is given by the second one:
\begin{gather*}
        t
    \bangArrSet_F
        (\app{x}{y})\esub{y}{\oc(z\esub{z}{\oc \oc (\app{I}{w})})}
    \bangArrSet_S
       \app{x}{(z\esub{z}{\oc \oc (\app{I}{w})})}
    \bangArrSet_F
       \app{x}{(z\esub{z}{\oc \oc (z\esub{z}{w})})}
    \bangArrSet_S
       \app{x}{\oc(z\esub{z}{w})}
\\
       t
    \;\;\bangArrSet_S\;\;
       \app{x}{(\app{I}{\oc\oc(\app{I}{w})})}
    \;\;\bangArrSet_S\;\;
       \app{x}{(z\esub{z}{\oc\oc(\app{I}{w})})}
    \;\;\bangArrSet_S\;\;
       \app{x}{\oc(\app{I}{w})}
    \;\;\bangArrSet_F\;\;
       \app{x}{\oc(z\esub{z}{w})}
\end{gather*} 
\end{example}






\subsection{\CBNSymb Factorization}
\label{subsec:CBN Factorization}

To achieve factorization in \CBNSymb\ via the abstract method, we
should show the existence of an $SFS$, which necessitates proving
numerous commutations. We avoid these long proofs by choosing a
simpler projection approach from~\BANGSymb.

As seen in the previous section, we claim that \surface reduction
constitutes the significant part of \full reduction. Consequently, we
identify the \insignificant\ sub-relation, also referred to as the
internal reduction. The \CBNSymb internal contexts $\cbnICtxt \in
\cbnICtxtSet$ are \full \CBNSymb contexts with holes positioned in an
argument. Formally,
%
\begin{align*}
\emphasis{(\CBNSymb Interior Ctxts)}
& &
\cbnICtxt &\;\Coloneqq\; \app[\,]{t}{\cbnFCtxt}
\vsep t\esub{x}{\cbnFCtxt}
\vsep \cbnSCtxt^*\cbnCtxtPlug{\cbnICtxt}
& &
\text{with }
\cbnSCtxt^* \in \cbnSCtxtSet \setminus \{\Hole\}
\end{align*}	

%
\noindent
The \emphasis{\CBNSymb internal reduction} $\cbnArrSet_I$ is
the closure over all internal contexts $\cbnICtxt \in \cbnICtxtSet$ of
the rewrite rules \cbnSymbBeta and \cbnSymbSubs. For
example, $\app{(\abs{x}{x})}{\Hole}$ is an internal context, while $\Hole$ is not, thus $\app{(\abs{x}{x})}{(\app{(\abs{y}{z})}{t})} \cbnArrSet_I
\app{(\abs{x}{x})}{z} \not\cbnArrSet_I z$.

As in the case of surface reduction, the \CBNSymb one step simulation
and reverse simulation (\Cref{l:one-step-cnb,l:reverse-simulation-cbn})
can be specialized to the internal case and we can show that positions
of \CBNSymb and \BANGSymb internal redexes are mutually mapped. This
allows us to show in particular the following property. 

% \begin{restatable}{corollary}{RecCbnPropInternal}
%     \label{cor:cbn prop-internal}
%     Let $t, u \in \setCbnTerms$,
%     %and $u' \in \setBangTerms$.
%     then $t \cbnArrSet*_I u$ if and only if $\cbnToBangAGK{t}
%     \bangArrSet*_I \cbnToBangAGK{u}$.
%     % \begin{itemize}
%     % \item \textbf{(Stability)}: \hspace{1.86cm}%
%     %         $\cbnToBangAGK{t} \bangArrSet*_I u'%
%     %             \quad \Rightarrow \quad%
%     %         \exists\, u \in \setCbnTerms, \; \cbnToBangAGK{u} = u'$

%     % \item \textbf{(Normal Forms)}: \hspace{0.2cm}%
%     %         $t \text{ is a \cbnSetINF}%
%     %             \quad\Leftrightarrow\quad%
%     %         \cbnToBangAGK{t} \text{ is a \bangSetINF}$

%     % \item \textbf{(Simulations)}: \hspace{1.32cm}%
%     %         $t \cbnArrSet*_I u%
%     %             \quad \Leftrightarrow \quad%
%     %         \cbnToBangAGK{t} \bangArrSet*_I \cbnToBangAGK{u}$

%     %     Moreover, the number of $\cbnSymbBeta/\cbnSymbSubs$-steps on
%     %     the left matches the number of
%     %     $\bangSymbBeta/\bangSymbSubs$-steps on the right.
%     % \end{itemize}
% \end{restatable}
\begin{restatable}{corollary}{RecCbnPropInternal}
    \label{cor:cbn prop-internal}
    Let $t, u \in \setCbnTerms$  and $\cgiulio{u}{s}' \in \setBangTerms$. Then, 
    \begin{itemize}
    \item \textbf{(Stability)}: \cgiulio{\hspace{1.86cm}%
            $\cbnToBangAGK{t} \bangArrSet*_I \cgiulio{u}{s}'%
                \quad \Rightarrow \quad%
            \exists\, \cgiulio{u}{s} \in \setCbnTerms, \; \cbnToBangAGK{\cgiulio{u}{s}} = \cgiulio{u}{s}'$}
        {if $\cbnToBangAGK{t} \bangArrSet*_I s'$ then
        	there is $s \in \setCbnTerms$ such that $\cbnToBangAGK{s} = s'$.}

    \item \textbf{(Normal Forms)}: \cgiulio{\hspace{0.2cm}%
            $t \text{ is a \cbnSetINF}%
                \quad\Leftrightarrow\quad%
            \cbnToBangAGK{t} \text{ is a \bangSetINF}$}
        {$t \text{ is a \cbnSetINF}$ if and only if 
        	$\cbnToBangAGK{t}$ is a \bangSetINF.}

    \item \textbf{(Simulations)}: \cgiulio{\hspace{1.32cm}%
            $t \cbnArrSet*_I u%
                \quad \Leftrightarrow \quad%
            \cbnToBangAGK{t} \bangArrSet*_I \cbnToBangAGK{u}$
        
    
 Moreover, the number of $\cbnSymbBeta/\cbnSymbSubs$-steps on
the left matches the number of
$\bangSymbBeta/\bangSymbSubs$-steps on the right.}
        {$t \cbnArrSet*_I u$ if and only if
        	$\cbnToBangAGK{t} \bangArrSet*_I \cbnToBangAGK{u}$.  
        	Moreover, the number of $\cbnSymbBeta/\cbnSymbSubs$-steps on
        	the left matches the number of
        	$\bangSymbBeta/\bangSymbSubs$-steps on the right.}
    \end{itemize}
\end{restatable}

\noindent
Via \Cref{cor:cbn prop-surface,cor:cbn prop-internal}, we can project
factorization from \BANGSymb back~to~\CBNSymb.

\begin{theorem}[\CBNSymb Factorization]
    \quad $\cbnArrSet*_F \;=\; \cbnArrSet*_S\cbnArrSet*_I$.
\end{theorem}
\begin{proof}
    The proof is depicted in \Cref{fig:proof cbn factorization}. In
    particular, since $\cbnToBangAGK{t} \bangArrSet*_S s'$, one
    deduces using \Cref{cor:cbn prop-surface} that there exists $s \in
    \setCbnTerms$ such that $\cbnToBangAGK{s} = s'$.
   \qed
\end{proof}

%% Ovalbox autour de la figure
\begin{figure}[t]
%  \ovalbox{
    \begin{minipage}[c]{0.49\textwidth}%
        \begin{tikzpicture}
            \node (0_t) at (-2.5, 0)      {$t$};
            \node (0_u) at (2.5, 0)       {$u$};

            \draw[->] (0_t) to ([xshift=-0.5cm]0_u);
            \node at ([xshift=-0.4cm, yshift=0.1cm]0_u) {*};
            \node at ([xshift=-0.35cm, yshift=-0.15cm]0_u) {$\scriptstyle\cbnFCtxtSet$};
            \node[rotate=-90] at (-0.65, -0.3)               {$\rightsquigarrow$};
            \node at (0, -0.3) {\scriptsize({\tt Cor.}\ref{cor:cbn prop-full})};

            \node (1_t) at (-2.5, -0.6)      {$\cbnToBangAGK{t}$};
            \node (1_u) at (2.5, -0.6)       {$\cbnToBangAGK{u}$};

            \draw[->] (1_t) to ([xshift=-0.6cm]1_u);
            \node at ([xshift=-0.5cm, yshift=0.1cm]1_u) {*};
            \node at ([xshift=-0.5cm, yshift=-0.15cm]1_u) {$\scriptstyle\bangFCtxtSet$};
            \node[rotate=-90] at (-0.65, -0.9)               {$\rightsquigarrow$};
            \node at (0, -0.9) {\scriptsize({\tt Cor.}\ref{lem:Bang_Factorization})};

            \node (2_t) at (-2.5, -1.2)      {$\cbnToBangAGK{t}$};
            \node (2_s) at (0, -1.2)         {$s'$};
            \node (2_u) at (2.5, -1.2)       {$\cbnToBangAGK{u}$};

            \draw[->] (2_t) to ([xshift=-0.4cm]2_s);
            \node at ([xshift=-0.3cm, yshift=0.1cm]2_s) {*};
            \node at ([xshift=-0.3cm, yshift=-0.15cm]2_s) {$\scriptstyle\bangSCtxtSet$};
            \draw[->] (2_s) to ([xshift=-0.6cm]2_u);
            \node at ([xshift=-0.5cm, yshift=0.1cm]2_u) {*};
            \node at ([xshift=-0.5cm, yshift=-0.15cm]2_u) {$\scriptstyle\bangICtxtSet$};
            \node[rotate=-90] at (-1.85, -1.5)               {$\rightsquigarrow$};
            \node at (-1.2, -1.5) {\scriptsize({\tt Cor.}\ref{cor:cbn prop-surface})};
            \node[rotate=-90] at (0.55, -1.5)               {$\rightsquigarrow$};
            \node at (1.2, -1.5) {\scriptsize({\tt Cor.}\ref{cor:cbn prop-internal})};

            % \node at (4.5, -2) {$(\cbnToBangAGK{s} = s')$};

            \node (3_t) at (-2.5, -1.8)      {$t$};
            \node (3_s) at (0, -1.8)         {$s$};
            \node (3_u) at (2.5, -1.8)       {$u$};

            \draw[->] (3_t) to ([xshift=-0.4cm]3_s);
            \node at ([xshift=-0.3cm, yshift=0.1cm]3_s) {*};
            \node at ([xshift=-0.25cm, yshift=-0.15cm]3_s) {$\scriptstyle\cbnSCtxtSet$};
            \draw[->] (3_s) to ([xshift=-0.4cm]3_u);
            \node at ([xshift=-0.3cm, yshift=0.1cm]3_u) {*};
            \node at ([xshift=-0.25cm, yshift=-0.15cm]3_u) {$\scriptstyle\cbnICtxtSet$};
        \end{tikzpicture}
        \vspace{-0.3cm}
        \caption{\CBNSymb factorization (with $s' \!=\! \cbnToBangAGK{s}$)}
        \label{fig:proof cbn factorization}
    \end{minipage}
\hspace{.5cm}
    \begin{minipage}[c]{0.49\textwidth}%
        \begin{tikzpicture}
            \node (0_t) at (-2.5, 0)      {$t$};
            \node (0_u) at (2.5, 0)       {$u$};

            \draw[->] (0_t) to ([xshift=-0.5cm]0_u);
            \node at ([xshift=-0.4cm, yshift=0.1cm]0_u) {*};
            \node at ([xshift=-0.35cm, yshift=-0.15cm]0_u) {$\scriptstyle\cbvFCtxtSet$};
            \node[rotate=-90] at (-0.65, -0.3)               {$\rightsquigarrow$};
            \node at (0, -0.3) {\scriptsize({\tt Cor.}\ref{cor:cbv prop-full})};

            \node (1_t) at (-2.5, -0.6)      {$\cbvToBangAGK{t}$};
            \node (1_u) at (2.5, -0.6)       {$\cbvToBangAGK{u}$};

            \draw[->] (1_t) to ([xshift=-0.6cm]1_u);
            \node at ([xshift=-0.5cm, yshift=0.1cm]1_u) {*};
            \node at ([xshift=-0.5cm, yshift=-0.15cm]1_u) {$\scriptstyle\bangFCtxtSet$};
            \node[rotate=-90] at (-0.65, -0.9)               {$\rightsquigarrow$};
            \node at (0, -0.9) {\scriptsize({\tt Cor.}\ref{lem:Bang_Factorization})};

            \node (2_t) at (-2.5, -1.2)      {$\cbvToBangAGK{t}$};
            \node (2_s) at (0, -1.2)         {$s'$};
            \node (2_u) at (2.5, -1.2)       {$\cbvToBangAGK{u}$};

            \draw[->] (2_t) to ([xshift=-0.4cm]2_s);
            \node at ([xshift=-0.3cm, yshift=0.1cm]2_s) {*};
            \node at ([xshift=-0.3cm, yshift=-0.15cm]2_s) {$\scriptstyle\bangSCtxtSet$};
            \draw[->] (2_s) to ([xshift=-0.6cm]2_u);
            \node at ([xshift=-0.5cm, yshift=0.1cm]2_u) {*};
            \node at ([xshift=-0.5cm, yshift=-0.15cm]2_u) {$\scriptstyle\bangICtxtSet$};
            \node[rotate=-90] at (-1.85, -1.5)               {$\rightsquigarrow$};
            \node at (-1.2, -1.5) {\scriptsize({\tt Cor.}\ref{cor:cbv prop-surface})};
            \node[rotate=-90] at (0.55, -1.5)               {$\rightsquigarrow$};
            \node at (1.2, -1.5) {\scriptsize({\tt Cor.}\ref{cor:cbv prop-internal})};

            % \node at (4.5, -2) {$(\cbvToBangAGK{s} = s')$};

            \node (3_t) at (-2.5, -1.8)      {$t$};
            \node (3_s) at (0, -1.8)         {$s$};
            \node (3_u) at (2.5, -1.8)       {$u$};

            \draw[->] (3_t) to ([xshift=-0.4cm]3_s);
            \node at ([xshift=-0.3cm, yshift=0.1cm]3_s) {*};
            \node at ([xshift=-0.25cm, yshift=-0.15cm]3_s) {$\scriptstyle\cbvSCtxtSet$};
            \draw[->] (3_s) to ([xshift=-0.4cm]3_u);
            \node at ([xshift=-0.3cm, yshift=0.1cm]3_u) {*};
            \node at ([xshift=-0.25cm, yshift=-0.15cm]3_u) {$\scriptstyle\cbvICtxtSet$};
        \end{tikzpicture}
        \vspace{-0.3cm}
        \caption{\CBVSymb factorization (with $s' \!=\! \cbvToBangAGK{s}$)}
        \label{fig:proof cbv factorization}
    \end{minipage}
%  }
\end{figure}













\subsection{\CBVSymb Factorization}
\label{subsec:CBV Factorization}

We now look at the more challenging case of projecting \BANGSymb
factorization back to \CBVSymb, eliminating the need for the extensive
commutation proofs required by the abstract method. Once again,
\CBVSymb surface reduction is considered to be the significant part of
\CBVSymb full reduction, so that we need to properly define the
\insignificant\  reduction, that we call \CBVSymb internal. The \CBVSymb
internal contexts $\cbvICtxt \in \cbvICtxtSet$ are full \CBVSymb
contexts with holes positioned under a lambda. Formally,
%
\begin{align*}
		\emphasis{(\CBVSymb Internal Ctxts)}
		& &
		\cbvICtxt&\;\Coloneqq\; \abs{x}{\cbvFCtxt}
		\vsep \cbvSCtxt^*\cbvCtxtPlug{\cbvICtxt}
		& &
		\text{with }
		\cbvSCtxt^* \in \cbvSCtxtSet \setminus \{\Hole\}
\end{align*}
\noindent
The \emphasis{\CBVSymb internal reduction} $\cbvArrSet_I$ is
the closure over all internal contexts $\cbvICtxt
\in \cbvICtxtSet$ of the rewrite rules \cbvSymbBeta and \cbvSymbSubs.
For example, $\app{(\abs{x}{\Hole})}{z}$ is an internal context while $\Hole$ is not, thus $\app{(\abs{x}{\app{(\abs{y}{y})}{z}})}{z}
\cbvArrSet_I \app{(\abs{x}{y\esub{y}{z}})}{z} \cbvArrSet_I
\app{(\abs{x}{z})}{z} \not\cbvArrSet_I z\esub{x}{z}$.

The \CBVSymb one step simulation and reverse simulation
(\Cref{lem:Cbv_Simulation_One_Step,lem:Cbv_Reverse_Simulation_One_Step})
can be specialized to the internal case, and we can easily show that
the positions of \CBVSymb and \BANGSymb internal redexes are mutually
mapped. Finally, diligence over the internal fragment allows to deduce
the following result:

% \begin{restatable}{corollary}{RecCbvPropInternal}
%     \label{cor:cbv prop-internal}
%     Let $t, u \in \setCbvTerms$,
%     % and $u' \in \setBangTerms$ such that $\bangPredINF<d!>{u'}$.
%     then $t \cbvArrSet*_I u$ if and only if $\cbvToBangAGK{t}
%     \bangArrSet*_I \cbvToBangAGK{u}$.
%     % \begin{itemize}
%     % \item \textbf{(Stability)}: \hspace{1.86cm}%
%     %         $\cbvToBangAGK{t} \bangArrSet*_I u'%
%     %             \quad \Rightarrow \quad%
%     %         \exists\, u \in \setCbvTerms, \; \cbvToBangAGK{u} = u'$

%     % \item \textbf{(Normal Forms)}: \hspace{0.2cm}%
%     %         $t \text{ is a \cbvSetINF}%
%     %             \quad\Leftrightarrow\quad%
%     %         \cbvToBangAGK{t} \text{ is a \bangSetINF}$

%     % \item \textbf{(Simulations)}: \hspace{1.32cm}%
%     %         $t \cbvArrSet*_I u%
%     %             \quad \Leftrightarrow \quad%
%     %         \cbvToBangAGK{t} \bangArrSet*_I \cbvToBangAGK{u}$

%     %         Moreover, the number of $\cbvSymbBeta/\cbvSymbSubs$-steps
%     %         on the left matches the number
%     %         $\bangSymbBeta/\bangSymbSubs$-steps on the right.
%     % \end{itemize}
% \end{restatable}
\begin{restatable}{corollary}{RecCbvPropInternal}
    \label{cor:cbv prop-internal}
    Let $t, u \in \setCbvTerms$ and $\cgiulio{u}{s}' \in \setBangTerms$\cgiulio{  such that
    $\bangPredINF<d!>{u'}$.}{.} Then,
    \begin{itemize}
    \item \textbf{(Stability)}: \cgiulio{\hspace{1.86cm}%
            $\cbvToBangAGK{t} \bangArrSet*_I \cgiulio{u}{s}'%
                \quad \Rightarrow \quad%
            \exists\, \cgiulio{u}{s} \in \setCbvTerms, \; \cbvToBangAGK{\cgiulio{u}{s}} = \cgiulio{u}{s}'$}
        {if $\cbvToBangAGK{t} \bangArrSet*_I \cgiulio{u}{s}'$ and $\bangPredINF<d!>{s'}$, then there is 
        $s \in \setCbvTerms$ such that $\cbvToBangAGK{s} = s'$.}

    \item \textbf{(Normal Forms)}: \cgiulio{\hspace{0.2cm}%
            $t \text{ is a \cbvSetINF}%
                \quad\Leftrightarrow\quad%
            \cbvToBangAGK{t} \text{ is a \bangSetINF}$}
        {$t \text{ is a \cbvSetINF}$ if and only if
        	$\cbvToBangAGK{t} \text{ is a \bangSetINF}$.}

    \item \textbf{(Simulations)}: \cgiulio{\hspace{1.32cm}%
            $t \cbvArrSet*_I u%
                \quad \Leftrightarrow \quad%
            \cbvToBangAGK{t} \bangArrSet*_I \cbvToBangAGK{u}$

            Moreover, the number of $\cbvSymbBeta/\cbvSymbSubs$-steps
            on the left matches the number
            $\bangSymbBeta/\bangSymbSubs$-steps on the right.}
        {$t \cbvArrSet*_I u$ if and only if 
        	$\cbvToBangAGK{t} \bangArrSet*_I \cbvToBangAGK{u}$.
        	Moreover, the number of $\cbvSymbBeta/\cbvSymbSubs$-steps
        	on the left matches the number
        	$\bangSymbBeta/\bangSymbSubs$-steps on the right.}
    \end{itemize}
\end{restatable}

\noindent
Via \Cref{cor:cbv prop-surface,cor:cbv prop-internal}, we can project
factorization from \BANGSymb back~to~\CBVSymb.

\begin{theorem}[\CBVSymb Factorization]
    \quad $\cbvArrSet*_F \;= \; \cbvArrSet*_S\cbvArrSet*_I$.
\end{theorem}
\begin{proof}
    The proof is depicted in \Cref{fig:proof cbv factorization}. In
    particular, by construction $\cbvToBangAGK{u}$ is a
    \bangSetFNF<d!> and by induction on the length of $s' \bangArr*_I
    \cbvToBangAGK{u}$, one has that $s'$ is a \bangSetSNF<d!>. Using
    \Cref{cor:cbv prop-surface}, one deduces that there exists $s \in
    \setCbvTerms$ such that $\cbvToBangAGK{s} = s'$.
    \qed
\end{proof}



==> 5_Proofs.tex <==
\section{Proofs of \Cref{sec:Bang_CBN_CBV_Confluence} : \nameSectionV}

% \subsection{\BANGSymb Generalized Diamond Property}

% \RecBangGeneralizedDiamond*
% \begin{proof} \label{prf:Bang_Generalized_Diamond}%
%     \delia{[D: Je n'ai pas lu cette preuve]}
% \end{proof}





\subsection{\BANGSymb Confluence}

\victor{[V: Certainement plus simple en (diamant $d!$ et $dB$ puis
parallèle $s!$) + Hindley-Rosen]}

Confluence of the surface reduction can be found in
\cite{BucciarelliKesnerRiosViso20,BucciarelliKesnerRiosViso23}. In
order to show confluence of the full reduction, we applied Tait and
Martin-Löf method. \delia{[D: expliquer pourquoi, la full reduction ne
verifie pas un diagramme de diamand]} \victorTodo

Let us first define the parallel full reduction for the
\bangCalculusSymb-calculus.

\newcommand{\bangParFNameStyle}[1]{{\tt #1}}
\newcommand{\bangParFNameRefl}
    {\bangParFNameStyle{(refl)}}
\newcommand{\bangParFNameBeta}
    {\bangParFNameStyle{(dB)}}
\newcommand{\bangParFNameSubs}
    {\bangParFNameStyle{(s!)}}
\newcommand{\bangParFNameBang}
    {\bangParFNameStyle{(d!)}}
\newcommand{\bangParFNameAbs}
    {\bangParFNameStyle{(abs)}}
\newcommand{\bangParFNameApp}
    {\bangParFNameStyle{(app)}}
\newcommand{\bangParFNameEsub}
    {\bangParFNameStyle{(es)}}
\newcommand{\bangParFNameDer}
    {\bangParFNameStyle{(der)}}
\newcommand{\bangParFNameOc}
    {\bangParFNameStyle{(bg)}}
\newcommand{\bangParFNameHoleRefl}
    {\bangParFNameStyle{(refl_{\Hole})}}
\newcommand{\bangParFNameHoleEsub}
    {\bangParFNameStyle{(es_{\Hole})}}

\newcommand{\hypoBangParF}          [2]
    {\hypo{#1 \bangParArrF #2}}
\newcommand{\inferBangParFRefl}     [2]
    {\infer0[\scriptsize\!$\bangParFNameRefl$]{#1 \bangParArrF #2}}
\newcommand{\inferBangParFBeta}     [2]
    {\infer3[\scriptsize\!$\bangParFNameBeta$]{#1 \bangParArrF #2}}
\newcommand{\inferBangParFSubs}     [2]
    {\infer3[\scriptsize\!$\bangParFNameSubs$]{#1 \bangParArrF #2}}
\newcommand{\inferBangParFBang}     [2]
    {\infer2[\scriptsize\!$\bangParFNameBang$]{#1 \bangParArrF #2}}
\newcommand{\inferBangParFAbs}      [2]
    {\infer1[\scriptsize\!$\bangParFNameAbs$]{#1 \bangParArrF #2}}
\newcommand{\inferBangParFApp}      [2]
    {\infer2[\scriptsize\!$\bangParFNameApp$]{#1 \bangParArrF #2}}
\newcommand{\inferBangParFEsub}     [2]
    {\infer2[\scriptsize\!$\bangParFNameEsub$]{#1 \bangParArrF #2}}
\newcommand{\inferBangParFDer}      [2]
    {\infer1[\scriptsize\!$\bangParFNameDer$]{#1 \bangParArrF #2}}
\newcommand{\inferBangParFOc}       [2]
    {\infer1[\scriptsize\!$\bangParFNameOc$]{#1 \bangParArrF #2}}
\newcommand{\inferBangParFHoleRefl} [2]
    {\infer0[\scriptsize\!$\bangParFNameHoleRefl$]{#1 \bangParArrF
    #2}}
\newcommand{\inferBangParFHoleEsub}   [2]
    {\infer2[\scriptsize\!$\bangParFNameHoleEsub$]{#1 \bangParArrF
    #2}}

\begin{definition}
    \begin{equation*}
        \hspace{-1.5cm}\begin{array}{c}
            \begin{prooftree}
                \hypoBangParF
                    {t}
                    {t'}
                \hypoBangParF
                    {u}
                    {u'}
                \hypoBangParF
                    {\bangLCtxt}
                    {\bangLCtxt'}
                \inferBangParFBeta
                    {\app{\bangLCtxt\bangCtxtPlug{\abs{x}{t}}}{u}}
                    {\bangLCtxt'\bangCtxtPlug{t'\esub{x}{u'}}}
            \end{prooftree}
        \hspace{1cm}
            \begin{prooftree}
                \hypoBangParF
                    {t}
                    {t'}
                \hypoBangParF
                    {u}
                    {u'}
                \hypoBangParF
                    {\bangLCtxt}
                    {\bangLCtxt'}
                \inferBangParFSubs
                    {t\esub{x}{\bangLCtxt\bangCtxtPlug{\oc u}}}
                    {\bangLCtxt'\bangCtxtPlug{t'\isub{x}{u'}}}
            \end{prooftree}
        \hspace{1cm}
            \begin{prooftree}
                \hypoBangParF
                    {t}
                    {t'}
                \hypoBangParF
                    {\bangLCtxt}
                    {\bangLCtxt'}
                \inferBangParFBang
                    {\der{\bangLCtxt\bangCtxtPlug{\oc t}}}
                    {\bangLCtxt'\bangCtxtPlug{t'}}
            \end{prooftree}
        \\[0.75cm]
            \begin{prooftree}
                \hypoBangParF
                    {t}
                    {t'}
                \inferBangParFAbs
                    {\abs{x}{t}}
                    {\abs{x}{t'}}
            \end{prooftree}
        \hspace{1cm}
            \begin{prooftree}
                \hypoBangParF
                    {t}
                    {t'}
                \hypoBangParF
                    {u}
                    {u'}
                \inferBangParFApp
                    {\app{t}{u}}
                    {\app{t'}{u'}}
            \end{prooftree}
        \hspace{1cm}
            \begin{prooftree}
                \hypoBangParF
                    {t}
                    {t'}
                \hypoBangParF
                    {u}
                    {u'}
                \inferBangParFEsub
                    {t\esub{x}{u}}
                    {t'\esub{x}{u'}}
            \end{prooftree}
        \hspace{1cm}
            \begin{prooftree}
                \hypoBangParF
                    {t}
                    {t'}
                \inferBangParFDer
                    {\der{t}}
                    {\der{t'}}
            \end{prooftree}
        \\[0.75cm]
            \begin{prooftree}
                \hypoBangParF
                    {t}
                    {t'}
                \inferBangParFOc
                    {\oc t}
                    {\oc t'}
            \end{prooftree}
        \hspace{1cm}
            \begin{prooftree}
                \inferBangParFRefl
                    {t}
                    {t}
            \end{prooftree}
        \hspace{1cm}
            \begin{prooftree}
                \inferBangParFHoleRefl
                    {\Hole}
                    {\Hole}
            \end{prooftree}
        \hspace{1cm}
            \begin{prooftree}
                \hypoBangParF
                    {\bangLCtxt}
                    {\bangLCtxt'}
                \hypoBangParF
                    {t}
                    {t'}
                \inferBangParFHoleEsub
                    {\bangLCtxt\esub{x}{t}}
                    {\bangLCtxt'\esub{x}{t'}}
            \end{prooftree}
        \end{array}
    \end{equation*}
\end{definition}


\begin{lemma}
    \label{lem: R in {dB, s!, d!} and t |->R u => t =-=> u} Let $t, u \in
    \setBangTerms$ and $\rel \in \{\bangSymbBeta, \bangSymbSubs,
    \bangSymbBang\}$ such that $t \mapstoR u$, then $t \bangParArrF
    u$.
\end{lemma}
\begin{proof}
  \deliaLu
  We distinguish three cases:
\begin{itemize}
\item[\bltI] $\rel = \bangSymbBeta$: Then $t =
    \app{\bangLCtxt\bangCtxtPlug{\abs{x}{s_1}}}{s_2}$ and $u =
    \bangLCtxt\bangCtxtPlug{s_1\esub{x}{s_2}}$: By induction on
    $\bangLCtxt$, one has that $\bangLCtxt \bangParArrF \bangLCtxt$
    \delia{ce commentaire apparait trois fois, l'ecrire une seule fois au debut de la preuve}Lemma 24
    thus:
    \begin{equation*}
        \begin{prooftree}
            \inferBangParFRefl
                {\abs{x}{s_1}}
                {\abs{x}{s_1}}
            \inferBangParFRefl
                {s_2}
                {s_2}
            \hypoBangParF
                {\bangLCtxt}
                {\bangLCtxt}
            \inferBangParFBeta
                {\app{\bangLCtxt\bangCtxtPlug{\abs{x}{s_1}}}{s_2}}
                {\bangLCtxt\bangCtxtPlug{s_1\esub{x}{s_2}}}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\rel = \bangSymbSubs$: Then $t =
    s_1\esub{x}{\bangLCtxt\bangCtxtPlug{\oc s_2}}$ and $u =
    \bangLCtxt\bangCtxtPlug{s_1\isub{x}{s_2}}$: By induction on
    $\bangLCtxt$, one has that $\bangLCtxt \bangParArrF \bangLCtxt$
    thus:
    \begin{equation*}
        \begin{prooftree}
            \inferBangParFRefl
                {s_1}
                {s_1}
            \inferBangParFRefl
                {\oc s_2}
                {\oc s_2}
            \hypoBangParF
                {\bangLCtxt}
                {\bangLCtxt}
            \inferBangParFSubs
                {s_1\esub{x}{\bangLCtxt\bangCtxtPlug{\oc s_2}}}
                {\bangLCtxt\bangCtxtPlug{s_1\isub{x}{s_2}}}
        \end{prooftree}
    \end{equation*}

\item[\bltI] $\rel = \bangSymbBang$: Then $t =
    \der{\bangLCtxt\bangCtxtPlug{\oc s'}}$ and $u =
    \bangLCtxt\bangCtxtPlug{s'}$: By induction on $\bangLCtxt$, one
    has that $\bangLCtxt \bangParArrF \bangLCtxt$ thus:
    \begin{equation*}
        \begin{prooftree}
            \inferBangParFRefl
                {\oc s'}
                {\oc s'}
            \hypoBangParF
                {\bangLCtxt}
                {\bangLCtxt}
            \inferBangParFBang
                {\der{\bangLCtxt\bangCtxtPlug{\oc s'}}}
                {\bangLCtxt\bangCtxtPlug{s'}}
        \end{prooftree}
    \end{equation*}

\end{itemize}
\end{proof}


\begin{lemma}
    \label{lem: t ->*F u => F<t> ->*F F<u>}
    Let $t, u \in \setBangTerms$ such that $t \bangArrsF u$. Then for
    any context $\bangFCtxt$, one has that $\bangFCtxt\bangCtxtPlug{t}
    \bangArrsF \bangFCtxt\bangCtxtPlug{u}$. \delia{[D: dans ce
    statement le F du contexte et le F de la reduction ont le meme
    nom et ceci est confus, surtout quand on change de contexte]}
\end{lemma}
\delia{ce lemme est trivial, je le mettrais comme une remarque seulement}

\begin{proof}
Let us proceed by induction on $t \bangArrsF u$:
\begin{itemize}
\item[\bltI] $t \bangArr^{0}_F u$: Then $t = u$ thus
    $\bangFCtxt\bangCtxtPlug{t} = \bangFCtxt\bangCtxtPlug{u}$ and by
    reflexivity $\bangFCtxt\bangCtxtPlug{t} \bangArrsF
    \bangFCtxt\bangCtxtPlug{u}$.

\item[\bltI] $t \bangArr_F s \bangArr^{n-1}_F u$: Since $t \bangArrF
    s$, then there exist $t', s' \in \setBangTerms$ such that $t =
    \bangFCtxt'\bangCtxtPlug{t'}$ and $s =
    \bangFCtxt'\bangCtxtPlug{u'}$ with $t' \mapstoR s'$ for some $\rel
    \in \{\bangSymbBeta, \bangSymbSubs, \bangSymbBang\}$. In
    particular, by considering the context
    $\bangFCtxt\bangCtxtPlug{\bangFCtxt'}$, one deduces that
    $\bangFCtxt\bangCtxtPlug{t} \bangArrF \bangFCtxt\bangCtxtPlug{s}$.
    By \ih on $s \bangArr^{n-1}_F u$, one obtains that
    $\bangFCtxt\bangCtxtPlug{s} \bangArrsF \bangFCtxt\bangCtxtPlug{u}$
    thus $\bangFCtxt\bangCtxtPlug{t} \bangArrsF
    \bangFCtxt\bangCtxtPlug{u}$ by transitivity.
\end{itemize}
\end{proof}


\begin{lemma}
    One has $\bangArrF \;\subseteq\; \bangParArrF \;\subseteq\;
    \bangArrsF$.
\end{lemma}
\begin{proof} \delia{[D: meme commentaire de confusion entre la F de
      la reduction et la F du contexte]}
  \deliaLu  \delia{mais c'est assez standard quand meme}
  We first prove the inclusion of the
left hand side and then follow with the intuition of the right hand
side:
\begin{itemize}
\item[$\bullet$] $\bangArrF \;\subseteq\; \bangParArrF$: Let $t
    \bangArrF u$ then there exists $t', u' \in \setBangTerms$ and
    $\bangFCtxt$ such that $t = \bangFCtxt\bangCtxtPlug{t}$, $u =
    \bangFCtxt\bangCtxtPlug{u'}$ and $t'
    \mapstoR[\bangFCtxt\bangCtxtPlug{\rel}] u'$ for $\rel \in
    \{\bangSymbBeta, \bangSymbSubs, \bangSymbBang\}$. Let us proceed
    by induction on $\bangFCtxt$:
    \begin{itemize}
    \item[\bltI] $\bangFCtxt = \Hole$: Then $t \mapstoR u$ and we
        conclude using \Cref{lem: R in {dB, s!, d!} and t |->R u => t =-=> u}.

    \item[\bltI] $\bangFCtxt = \abs{x}{\bangFCtxt'}$: Since
        $\bangFCtxt'\bangCtxtPlug{t'} \bangArrF
        \bangFCtxt'\bangCtxtPlug{u'}$, by \ih on $\bangFCtxt'$, one
        deduces that $\bangFCtxt'\bangCtxtPlug{t'} \bangParArrF
        \bangFCtxt'\bangCtxtPlug{u'}$ which concludes this case since:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {\bangFCtxt'\bangCtxtPlug{t'}}
                    {\bangFCtxt'\bangCtxtPlug{u'}}
                \inferBangParFAbs
                    {\abs{x}{\bangFCtxt'\bangCtxtPlug{t'}}}
                    {\abs{x}{\bangFCtxt'\bangCtxtPlug{u'}}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangFCtxt = \app{\bangFCtxt'}{s}$: Since
        $\bangFCtxt'\bangCtxtPlug{t'} \bangArrF
        \bangFCtxt'\bangCtxtPlug{u'}$, by \ih on $\bangFCtxt'$, one
        deduces that $\bangFCtxt'\bangCtxtPlug{t'} \bangParArrF
        \bangFCtxt'\bangCtxtPlug{u'}$ which concludes this case since:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {\bangFCtxt'\bangCtxtPlug{t'}}
                    {\bangFCtxt'\bangCtxtPlug{u'}}
                \inferBangParFRefl
                    {s}
                    {s}
                \inferBangParFApp
                    {\app{\bangFCtxt'\bangCtxtPlug{t'}}{s}}
                    {\app{\bangFCtxt'\bangCtxtPlug{u'}}{s}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangFCtxt = \app[\,]{s}{\bangFCtxt'}$: Since
        $\bangFCtxt'\bangCtxtPlug{t'} \bangArrF
        \bangFCtxt'\bangCtxtPlug{u'}$, by \ih on $\bangFCtxt'$, one
        deduces that $\bangFCtxt'\bangCtxtPlug{t'} \bangParArrF
        \bangFCtxt'\bangCtxtPlug{u'}$ which concludes this case since:
        \begin{equation*}
            \begin{prooftree}
                \inferBangParFRefl
                    {s}
                    {s}
                \hypoBangParF
                    {\bangFCtxt'\bangCtxtPlug{t'}}
                    {\bangFCtxt'\bangCtxtPlug{u'}}
                \inferBangParFApp
                    {\app[\,]{s}{\bangFCtxt'\bangCtxtPlug{t'}}}
                    {\app[\,]{s}{\bangFCtxt'\bangCtxtPlug{u'}}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangFCtxt = \bangFCtxt'\esub{x}{s}$: Since
        $\bangFCtxt'\bangCtxtPlug{t'} \bangArrF
        \bangFCtxt'\bangCtxtPlug{u'}$, by \ih on $\bangFCtxt'$, one
        deduces that $\bangFCtxt'\bangCtxtPlug{t'} \bangParArrF
        \bangFCtxt'\bangCtxtPlug{u'}$ which concludes this case since:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {\bangFCtxt'\bangCtxtPlug{t'}}
                    {\bangFCtxt'\bangCtxtPlug{u'}}
                \inferBangParFRefl
                    {s}
                    {s}
                \inferBangParFEsub
                    {\bangFCtxt'\bangCtxtPlug{t'}\esub{s}}
                    {\bangFCtxt'\bangCtxtPlug{u'}\esub{x}{s} \delia{\mbox{typo a gauche}}} 
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangFCtxt = s\esub{x}{\bangFCtxt'}$: Since
        $\bangFCtxt'\bangCtxtPlug{t'} \bangArrF
        \bangFCtxt'\bangCtxtPlug{u'}$, by \ih on $\bangFCtxt'$, one
        deduces that $\bangFCtxt'\bangCtxtPlug{t'} \bangParArrF
        \bangFCtxt'\bangCtxtPlug{u'}$ which concludes this case since:
        \begin{equation*}
            \begin{prooftree}
                \inferBangParFRefl
                    {s}
                    {s}
                \hypoBangParF
                    {\bangFCtxt'\bangCtxtPlug{t'}}
                    {\bangFCtxt'\bangCtxtPlug{u'}}
                \inferBangParFApp
                    {s\esub{x}{\bangFCtxt'\bangCtxtPlug{t'}}}
                    {s\esub{x}{\bangFCtxt'\bangCtxtPlug{u'}}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangFCtxt = \der{\bangFCtxt'}$: Since
        $\bangFCtxt'\bangCtxtPlug{t'} \bangArrF
        \bangFCtxt'\bangCtxtPlug{u'}$, by \ih on $\bangFCtxt'$, one
        deduces that $\bangFCtxt'\bangCtxtPlug{t'} \bangParArrF
        \bangFCtxt'\bangCtxtPlug{u'}$ which concludes this case since:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {\bangFCtxt'\bangCtxtPlug{t'}}
                    {\bangFCtxt'\bangCtxtPlug{u'}}
                \inferBangParFDer
                    {\der{\bangFCtxt'\bangCtxtPlug{t'}}}
                    {\der{\bangFCtxt'\bangCtxtPlug{u'}}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangFCtxt = \oc\bangFCtxt'$: Since
        $\bangFCtxt'\bangCtxtPlug{t'} \bangArrF
        \bangFCtxt'\bangCtxtPlug{u'}$, by \ih on $\bangFCtxt'$, one
        deduces that $\bangFCtxt'\bangCtxtPlug{t'} \bangParArrF
        \bangFCtxt'\bangCtxtPlug{u'}$ which concludes this case since:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {\bangFCtxt'\bangCtxtPlug{t'}}
                    {\bangFCtxt'\bangCtxtPlug{u'}}
                \inferBangParFOc
                    {\oc{\bangFCtxt'\bangCtxtPlug{t'}}}
                    {\oc{\bangFCtxt'\bangCtxtPlug{u'}}}
            \end{prooftree}
        \end{equation*}
    \end{itemize}

\item[$\bullet$] $\bangParArrF \;\subseteq\; \bangArrsF$: Consider the
    following stronger statement:
    \begin{enumerate}
    \item If $t \bangParArrF u$ then $t \bangArrsF u$.
    \item If $\bangLCtxt \bangParArrF \bangLCtxt'$ then for any $t \in
        \setBangTerms$, one has $\bangLCtxt\bangCtxtPlug{t} \bangArrsF
        \bangLCtxt'\bangCtxtPlug{t}$.
    \end{enumerate}

    We proceed by simultaneous induction on $t \bangParArrF u$ and
    $\bangLCtxt \bangParArrF \bangLCtxt'$.
    \begin{enumerate}
    \item We consider the following cases:
        \begin{itemize}
        \item[\bltI] $\bangParFNameBeta$: Then there exist terms $s_1,
            s'_1, s_2, s'_2 \in \setBangTerms$ and context
            $\bangLCtxt, \bangLCtxt'$ such that $t =
            \app{\bangLCtxt\bangCtxtPlug{\abs{x}{s_1}}}{s_2}$ and $u =
            \bangLCtxt'\bangCtxtPlug{s'_1\esub{x}{s'_2}}$ and so that
            the statement has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s_1}
                        {s'_1}
                    \hypoBangParF
                        {s_2}
                        {s'_2}
                    \hypoBangParF
                        {\bangLCtxt}
                        {\bangLCtxt'}
                    \inferBangParFBeta
                        {\app{\bangLCtxt\bangCtxtPlug{\abs{x}{s_1}}}{s_2}}
                        {\bangLCtxt'\bangCtxtPlug{s'_1\esub{x}{s'_2}}}
                \end{prooftree}
            \end{equation*}
            By \ih (2) on $\bangLCtxt \bangParArrF \bangLCtxt'$, one
            has that $\bangLCtxt\bangCtxtPlug{\abs{x}{s_1}} \bangArrsF
            \bangLCtxt'\bangCtxtPlug{\abs{x}{s_1}}$. By \ih (1) on
            $s_1 \bangParArrF s'_1$ and $s_2 \bangParArrF s'_2$, one
            obtains that $s_1 \bangArrsF s'_1$ and $s_2 \bangArrsF
            s'_2$. Using \Cref{lem: t ->*F u => F<t> ->*F F<u>} on
            $s_1 \bangArrsF s'_1$ with $\app{\bangLCtxt'}{s_2}$, one
            deduces that
            $\app{\bangLCtxt'\bangCtxtPlug{\abs{x}{s_1}}}{s_2}
            \bangArrsF
            \app{\bangLCtxt'\bangCtxtPlug{\abs{x}{s'_1}}}{s_2}$.
            Similarly, using again \Cref{lem: t ->*F u => F<t> ->*F
            F<u>} on $s_2 \bangArrsF s'_2$ with
            $\app{\bangLCtxt'\bangCtxtPlug{\abs{x}{s'_1}}}{\Hole}$,
            one deduces that
            $\app{\bangLCtxt'\bangCtxtPlug{\abs{x}{s'_1}}}{s_2}
            \bangArrsF
            \app{\bangLCtxt'\bangCtxtPlug{\abs{x}{s'_1}}}{s'_2}$.
            Finally, one has that
            $\app{\bangLCtxt'\bangCtxtPlug{\abs{x}{s'_1}}}{s'_2}
            \bangArrF \bangLCtxt'\bangCtxtPlug{s'_1\esub{x}{s'_2}}$
            and thus $\app{\bangLCtxt\bangCtxtPlug{\abs{x}{s_1}}}{s_2}
            \bangArrsF \bangLCtxt'\bangCtxtPlug{s'_1\esub{x}{s'_2}}$
            by transitivity.

        \item[\bltI] $\bangParFNameSubs$: Then there exist terms $s_1,
            s'_1, s_2, s'_2 \in \setBangTerms$ and contexts
            $\bangLCtxt, \bangLCtxt'$ such that $t =
            s_1\esub{x}{\bangLCtxt\bangCtxtPlug{\oc s_2}}$ and $u =
            \bangLCtxt'\bangCtxtPlug{s'_1\isub{x}{s'_2}}$ and so that
            the statement has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s_1}
                        {s'_1}
                    \hypoBangParF
                        {s_2}
                        {s'_2}
                    \hypoBangParF
                        {\bangLCtxt}
                        {\bangLCtxt'}
                    \inferBangParFSubs
                        {s_1\esub{x}{\bangLCtxt\bangCtxtPlug{\oc s_2}}}
                        {\bangLCtxt'\bangCtxtPlug{s'_1\isub{x}{s'_2}}}
                \end{prooftree}
            \end{equation*}
            By \ih (2) on $\bangLCtxt \bangParArrF \bangLCtxt'$, one
            has that $s_1\esub{x}{\bangLCtxt\bangCtxtPlug{\oc s_2}}
            \bangArrsF s_1\esub{x}{\bangLCtxt'\bangCtxtPlug{\oc
            s_2}}$. By \ih (1) on $s_1 \bangParArrF s'_1$ and $s_2
            \bangParArrF s'_2$, one obtains that $s_1 \bangArrsF s'_1$
            and $s_2 \bangArrsF s'_2$. Using \Cref{lem: t ->*F u =>
            F<t> ->*F F<u>} on $s_1 \bangArrsF s'_1$ with
            $\Hole\esub{x}{\bangLCtxt'\bangCtxtPlug{\oc s_2}}$, one
            deduces that $s_1\esub{x}{\bangLCtxt'\bangCtxtPlug{\oc
            s_2}} \bangArrsF s'_1\esub{x}{\bangLCtxt'\bangCtxtPlug{\oc
            s_2}}$. Similarly, using again \Cref{lem: t ->*F u => F<t>
            ->*F F<u>} on $s_2 \bangArrsF s'_2$ with
            $s'_1\esub{x}{\bangLCtxt'\bangCtxtPlug{\Hole}}$, one
            deduces that $s'_1\esub{x}{\bangLCtxt'\bangCtxtPlug{\oc
            s_2}} \bangArrsF s'_1\esub{x}{\bangLCtxt'\bangCtxtPlug{\oc
            s'_2}}$. Finally, one has that
            $\bangLCtxt'\bangCtxtPlug{s_1\isub{x}{s_2}} \bangArrF
            \bangLCtxt'\bangCtxtPlug{s'_1\isub{x}{s'_2}}$ and thus
            $s_1\esub{x}{\bangLCtxt\bangCtxtPlug{\oc s_2}} \bangArrsF
            \bangLCtxt'\bangCtxtPlug{s'_1\isub{x}{s'_2}}$ by
            transitivity.

        \item[\bltI] $\bangParFNameBang$: Then there exist terms $s,
            s' \in \setBangTerms$ and contexts $\bangLCtxt,
            \bangLCtxt'$ such that $t =
            \der{\bangLCtxt\bangCtxtPlug{\oc s}}$ and $u =
            \bangLCtxt'\bangCtxtPlug{s'}$ and so that the statement
            has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s}
                        {s'}
                    \hypoBangParF
                        {\bangLCtxt}
                        {\bangLCtxt'}
                    \inferBangParFBang
                        {\der{\bangLCtxt\bangCtxtPlug{\oc s}}}
                        {\bangLCtxt'\bangCtxtPlug{s'}}
                \end{prooftree}
            \end{equation*}
            By \ih (2) on $\bangLCtxt \bangParArrF \bangLCtxt'$, one
            has that $\der{\bangLCtxt\bangCtxtPlug{\oc s}} \bangArrsF
            \der{\bangLCtxt'\bangCtxtPlug{\oc s}}$. By \ih (1) on $s
            \bangParArrF s'$ and using \Cref{lem: t ->*F u => F<t>
            ->*F F<u>} on $s_1 \bangArrsF s'_1$ with
            $\der{\bangLCtxt'\bangCtxtPlug{\oc \Hole}}$, one deduces
            that $\der{\bangLCtxt'\bangCtxtPlug{\oc s}} \bangArrsF
            \der{\bangLCtxt'\bangCtxtPlug{\oc s'}}$. Since
            $\der{\bangLCtxt'\bangCtxtPlug{\oc s'}} \bangArrF
            \bangLCtxt'\bangCtxtPlug{s'}$ then one concludes that
            $\der{\bangLCtxt\bangCtxtPlug{\oc s}} \bangArrsF
            \bangLCtxt'\bangCtxtPlug{s'}$ by transitivity.

        \item[\bltI] $\bangParFNameAbs$: Then there exist $s, s' \in
            \setBangTerms$ such that $t = \abs{x}{s}$ and $u =
            \abs{x}{s'}$ and so that the statement has the following
            form:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s}
                        {s'}
                    \inferBangParFAbs
                        {\abs{x}{s}}
                        {\abs{x}{s'}}
                \end{prooftree}
            \end{equation*}
            By \ih (1) on $s \bangParArrF s'$ and using \Cref{lem: t
            ->*F u => F<t> ->*F F<u>} on $s \bangArrsF s'$ with
            $\abs{x}{\Hole}$, one concludes that $\abs{x}{s}
            \bangArrsF \abs{x}{s'}$.

        \item[\bltI] $\bangParFNameApp$: Then there exist $s_1, s'_1,
            s_2, s'_2 \in \setBangTerms$ such that $t =
            \app{s_1}{s_2}$ and $u = \app{s'_1}{s'_2}$ and so that the
            statement has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s_1}
                        {s'_1}
                    \hypoBangParF
                        {s_2}
                        {s'_2}
                    \inferBangParFApp
                        {\app{s_1}{s_2}}
                        {\app{s'_1}{s'_2}}
                \end{prooftree}
            \end{equation*}
            By \ih (1) on $s_1 \bangParArrF s'_1$ and $s_2
            \bangParArrF s'_2$, one obtains that $s_1 \bangArrsF s'_1$
            and $s_2 \bangArrsF s'_2$. Using \Cref{lem: t ->*F u =>
            F<t> ->*F F<u>} on $s_1 \bangArrsF s'_1$ with
            $\app[\,]{\Hole}{s_2}$, one deduces that $\app{s_1}{s_2}
            \bangArrsF \app{s'_1}{s_2}$. Similarly, using again
            \Cref{lem: t ->*F u => F<t> ->*F F<u>} on $s_2 \bangArrsF
            s'_2$ with $\app{s'_1}{\Hole}$, one deduces that
            $\app{s'_1}{s_2} \bangArrsF \app{s'_1}{s'_2}$, thus
            $\app{s_1}{s_2} \bangArrsF \app{s'_1}{s'_2}$ by
            transitivity.

        \item[\bltI] $\bangParFNameEsub$: Then there exist $s_1, s'_1,
            s_2, s'_2 \in \setBangTerms$ such that $t =
            s_1\esub{x}{s_2}$ and $u = s'_1\esub{x}{s'_2}$ and so that
            the statement has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s_1}
                        {s'_1}
                    \hypoBangParF
                        {s_2}
                        {s'_2}
                    \inferBangParFEsub
                        {s_1\esub{x}{s_2}}
                        {s'_1\esub{x}{s'_2}}
                \end{prooftree}
            \end{equation*}
            By \ih (1) on $s_1 \bangParArrF s'_1$ and $s_2
            \bangParArrF s'_2$, one obtains that $s_1 \bangArrsF s'_1$
            and $s_2 \bangArrsF s'_2$. Using \Cref{lem: t ->*F u =>
            F<t> ->*F F<u>} on $s_1 \bangArrsF s'_1$ with
            $\Hole\esub{x}{s_2}$, one deduces that $s_1\esub{x}{s_2}
            \bangArrsF s'_1\esub{x}{s_2}$. Similarly, using again
            \Cref{lem: t ->*F u => F<t> ->*F F<u>} on $s_2 \bangArrsF
            s'_2$ with $s'_1\esub{x}{\Hole}$, one deduces that
            $s'_1\esub{x}{s_2} \bangArrsF s'_1\esub{x}{s'_2}$, thus
            $s_1\esub{x}{s_2} \bangArrsF s'_1\esub{x}{s'_2}$ by
            transitivity.

        \item[\bltI] $\bangParFNameDer$: Then there exist $s, s' \in
            \setBangTerms$ such that $t = \der{s}$ and $u = \der{s'}$
            and so that the statement has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s}
                        {s'}
                    \inferBangParFDer
                        {\der{s}}
                        {\der{s'}}
                \end{prooftree}
            \end{equation*}
            By \ih (1) on $s \bangParArrF s'$ and using
            \Cref{lem: t ->*F u => F<t> ->*F F<u>} on $s \bangArrsF
            s'$ with $\der{\Hole}$, one concludes that $\der{s}
            \bangArrsF \der{s'}$.

        \item[\bltI] $\bangParFNameOc$: Then there exist $s, s' \in
            \setBangTerms$ such that $t = \oc s$ and $u = \oc s'$ and
            so that the statement has the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s}
                        {s'}
                    \inferBangParFOc
                        {\oc s}
                        {\oc s'}
                \end{prooftree}
            \end{equation*}
            By \ih (1) on $s \bangParArrF s'$ and using \Cref{lem: t
            ->*F u => F<t> ->*F F<u>} on $s \bangArrsF s'$ with $\oc
            \Hole$, one concludes that $\oc s \bangArrsF \oc s'$.

        \item[\bltI] $\bangParFNameRefl$: Then $t = u$ and by
            reflexivity $t \bangArrsF u$.
        \end{itemize}

    \item We consider the following cases:
        \begin{itemize}
        \item[\bltI] $\bangParFNameHoleRefl$: Then $\bangLCtxt =
            \Hole$ and $\bangLCtxt' = \Hole$ thus
            $\bangLCtxt\bangCtxtPlug{t} = t$ and
            $\bangLCtxt'\bangCtxtPlug{t} = t$. We easily conclude $t
            \bangArrsF t $.

        \item[\bltI] $\bangParFNameHoleEsub$: Then $\bangLCtxt =
            \bangLCtxt_1\esub{x}{s}$, $\bangLCtxt' =
            \bangLCtxt'_1\esub{x}{s'}$ and so that the statement has
            the following form:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {\bangLCtxt_1}
                        {\bangLCtxt'_1}
                    \hypoBangParF
                        {s}
                        {s'}
                    \inferBangParFHoleEsub
                        {\bangLCtxt_1\esub{x}{s}}
                        {\bangLCtxt'_1\esub{x}{s'}}
                \end{prooftree}
            \end{equation*}
            By \ih (2) on $\bangLCtxt_1 \bangParArrF \bangLCtxt'_1$,
            one obtains that $\bangLCtxt_1\bangCtxtPlug{t} \bangArrsF
            \bangLCtxt'_1\bangCtxtPlug{t}$. Using \Cref{lem: t ->*F u
            => F<t> ->*F F<u>} with $\Hole\esub{x}{s}$, one has that
            $\bangLCtxt\bangCtxtPlug{t}\esub{x}{s} \bangArrsF
            \bangLCtxt\bangCtxtPlug{u}\esub{x}{s}$. By \ih (1) on $s
            \bangParArrF s'$, one has that $s \bangArrsF s'$ and using
            again \Cref{lem: t ->*F u => F<t> ->*F F<u>} with
            $\bangLCtxt\bangCtxtPlug{u}\esub{x}{\Hole}$, one deduces
            that $\bangLCtxt\bangCtxtPlug{u}\esub{x}{s} \bangArrsF
            \bangLCtxt\bangCtxtPlug{u}\esub{x}{s'}$ and we conclude
            that $\bangLCtxt\bangCtxtPlug{t}\esub{x}{s} \bangArrsF
            \bangLCtxt\bangCtxtPlug{u}\esub{x}{s'}$ by transitivity.
        \end{itemize}
    \end{enumerate}
\end{itemize}
\end{proof}


\begin{lemma}
    If $t \bangParArrF t'$ and $u \bangParArrF u'$ then $t\isub{x}{u}
    \bangParArrF t'\isub{x}{u'}$
\end{lemma}
\begin{proof}
  \deliaLu  \delia{mais c'est assez standard quand meme}
  Consider the following stronger statement:
\begin{enumerate}
\item If $t \bangParArrF t'$ and $u \bangParArrF u'$ then
    $t\isub{x}{u} \bangParArrF t'\isub{x}{u'}$
\item If $\bangLCtxt \bangParArrF \bangLCtxt'$ and $u \bangParArrF u'$
  then $\bangLCtxt\isub{x}{u} \bangParArrF \bangLCtxt'\isub{x}{u'}$.
  \delia{attention il faut definir la notion de $\bangLCtxt\isub{x}{u}$}
\end{enumerate}

We proceed by simultaneous induction on the statements $t \bangParArrF
t'$ and $\bangLCtxt \bangParArrF \bangLCtxt'$:
\begin{enumerate}
\item $t \bangParArrF u$: We distinguish $9$ different cases:
    \begin{itemize}
    \item[\bltI] $\bangParFNameBeta$: Then $t =
        \app{\bangLCtxt\bangCtxtPlug{\abs{y}{s_1}}}{s_2}$, $t' =
        \bangLCtxt'\bangCtxtPlug{s'_1\esub{x}{s'_2}}$ and the
        statement has the following form:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s_1}
                    {s'_1}
                \hypoBangParF
                    {s_2}
                    {s'_2}
                \hypoBangParF
                    {\bangLCtxt}
                    {\bangLCtxt'}
                \inferBangParFBeta
                    {\app{\bangLCtxt\bangCtxtPlug{\abs{y}{s_1}}}{s_2}}
                    {\bangLCtxt'\bangCtxtPlug{s'_1\esub{y}{s'_2}}}
            \end{prooftree}
        \end{equation*}
        By \ih (2) on $\bangLCtxt \bangParArrF \bangLCtxt'$, one has
        that $\bangLCtxt\isub{x}{u} \bangParArrF
        \bangLCtxt'\isub{x}{u'}$. Similarly, by \ih (1) on $s_1
        \bangParArrF s'_1$ and $s_2 \bangParArrF s'_2$, one obtains
        that $s_1\isub{x}{u} \bangParArrF s'_1\isub{x}{u'}$ and
        $s_2\isub{x}{u} \bangParArrF s'_2\isub{x}{u'}$. Since
        $t\isub{x}{u} =
        \app{\bangLCtxt\isub{x}{u}\bangCtxtPlug{\abs{y}{s_1\isub{x}{u}}}}{s_2\isub{x}{u}}$
        and $t'\isub{x}{u'} =
        \bangLCtxt\isub{x}{u'}\bangCtxtPlug{s'_1\isub{x}{u'}\esub{y}{s'_2\isub{x}{u'}}}$,
        one concludes this case as follows:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s_1\isub{x}{u}}
                    {s'_1\isub{x}{u'}}
                \hypoBangParF
                    {s_2\isub{x}{u}}
                    {s'_2\isub{x}{u'}}
                \hypoBangParF
                    {\bangLCtxt\isub{x}{u}}
                    {\bangLCtxt'\isub{x}{u'}}
                \inferBangParFBeta
                    {\app{\bangLCtxt\isub{x}{u}\bangCtxtPlug{\abs{y}{s_1\isub{x}{u}}}}{s_2\isub{x}{u}}}
                    {\bangLCtxt\isub{x}{u'}\bangCtxtPlug{s'_1\isub{x}{u'}\esub{y}{s'_2\isub{x}{u'}}}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangParFNameSubs$: Then $t =
        s_1\esub{y}{\bangLCtxt\bangCtxtPlug{\oc s_2}}$, $t' =
        \bangLCtxt'\bangCtxtPlug{s'_1\isub{y}{s'_2}}$ and the
        statement has the following form:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s_1}
                    {s'_1}
                \hypoBangParF
                    {s_2}
                    {s'_2}
                \hypoBangParF
                    {\bangLCtxt}
                    {\bangLCtxt'}
                \inferBangParFSubs
                    {s_1\esub{y}{\bangLCtxt\bangCtxtPlug{\oc s_2}}}
                    {\bangLCtxt'\bangCtxtPlug{s'_1\isub{y}{s'_2}}}
            \end{prooftree}
        \end{equation*}
        By \ih (2) on $\bangLCtxt \bangParArrF \bangLCtxt'$, one has
        that $\bangLCtxt\isub{x}{u} \bangParArrF
        \bangLCtxt'\isub{x}{u'}$. Similarly, by \ih (1) on $s_1
        \bangParArrF s'_1$ and $s_2 \bangParArrF s'_2$, one obtains
        that $s_1\isub{x}{u} \bangParArrF s'_1\isub{x}{u'}$ and
        $s_2\isub{x}{u} \bangParArrF s'_2\isub{x}{u'}$. Since
        $t\isub{x}{u} =
        s_1\isub{x}{u}\esub{y}{\bangLCtxt\isub{x}{u}\bangCtxtPlug{\oc
        s_2\isub{x}{u}}}$ and $t'\isub{x}{u'} =
        \bangLCtxt'\isub{x}{u'}\bangCtxtPlug{s'_1\isub{x}{u'}\isub{y}{s'_2\isub{x}{u'}}}$,
        one concludes this case as follows:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s_1\isub{x}{u}}
                    {s'_1\isub{x}{u'}}
                \hypoBangParF
                    {s_2\isub{x}{u}}
                    {s'_2\isub{x}{u'}}
                \hypoBangParF
                    {\bangLCtxt\isub{x}{u}}
                    {\bangLCtxt'\isub{x}{u'}}
                \inferBangParFSubs
                    {s_1\isub{x}{u}\esub{y}{\bangLCtxt\isub{x}{u}\bangCtxtPlug{\oc s_2\isub{x}{u}}}}
                    {\bangLCtxt'\isub{x}{u'}\bangCtxtPlug{s'_1\isub{x}{u'}\isub{y}{s'_2\isub{x}{u'}}}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangParFNameBang$: Then $t =
        \der{\bangLCtxt\bangCtxtPlug{\oc s}}$, $t' =
        \bangLCtxt'\bangCtxtPlug{s'}$ and the statement has the
        following form:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s}
                    {s'}
                \hypoBangParF
                    {\bangLCtxt}
                    {\bangLCtxt'}
                \inferBangParFBang
                    {\der{\bangLCtxt\bangCtxtPlug{\oc s}}}
                    {\bangLCtxt'\bangCtxtPlug{s'}}
            \end{prooftree}
        \end{equation*}
        By \ih (2) on $\bangLCtxt \bangParArrF \bangLCtxt'$, one has
        that $\bangLCtxt\isub{x}{u} \bangParArrF
        \bangLCtxt'\isub{x}{u'}$. Similarly, by \ih (1) on $s
        \bangParArrF s'$ one obtains that $s\isub{x}{u} \bangParArrF
        s'\isub{x}{u'}$. Since $t\isub{x}{u} =
        \der{\bangLCtxt\isub{x}{u}\bangCtxtPlug{\oc s\isub{x}{u}}}$
        and $t'\isub{x}{u'} =
        \bangLCtxt'\isub{x}{u'}\bangCtxtPlug{s'\isub{x}{u'}}$, one
        concludes this case as follows:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s\isub{x}{u}}
                    {s'\isub{x}{u'}}
                \hypoBangParF
                    {\bangLCtxt\isub{x}{u}}
                    {\bangLCtxt'\isub{x}{u'}}
                \inferBangParFBang
                    {\der{\bangLCtxt\isub{x}{u}\bangCtxtPlug{\oc s\isub{x}{u}}}}
                    {\bangLCtxt\isub{x}{u'}\bangCtxtPlug{s'\isub{x}{u'}}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangParFNameAbs$: Then there exist $s, s' \in
        \setBangTerms$ such that $t = \abs{y}{s}$ and $u =
        \abs{y}{s'}$ and so that the statement has the following form:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF{s}{s'}
                \inferBangParFAbs
                    {\abs{y}{s}}
                    {\abs{y}{s'}}
            \end{prooftree}
        \end{equation*}
        By \ih (1) on $s \bangParArrF s'$, one obtains that
        $s\isub{x}{u} \bangParArrF s'\isub{x}{u'}$. Since
        $t\isub{x}{u} = \abs{y}{s\isub{x}{u}}$ and $t'\isub{x}{u'} =
        \abs{y}{s'\isub{x}{u'}}$, one concludes this case as follows:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s\isub{x}{u}}
                    {s'\isub{x}{u'}}
                \inferBangParFAbs
                    {\abs{y}{s\isub{x}{u}}}
                    {\abs{y}{s'\isub{x}{u'}}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangParFNameApp$: Then there exist $s_1, s'_1, s_2,
        s'_2 \in \setBangTerms$ such that $t = \app{s_1}{s_2}$ and $u
        = \app{s'_1}{s'_2}$ and so that the statement has the
        following form:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s_1}
                    {s'_1}
                \hypoBangParF
                    {s_2}
                    {s'_2}
                \inferBangParFApp
                    {\app{s_1}{s_2}}
                    {\app{s'_1}{s'_2}}
            \end{prooftree}
        \end{equation*}
        By \ih (1) on $s_1 \bangParArrF s'_1$ and $s_2 \bangParArrF
        s'_2$, one obtains that $s_1\isub{x}{u} \bangParArrF
        s'_1\isub{x}{u'}$ and $s_2\isub{x}{u} \bangParArrF
        s'_2\isub{x}{u'}$. Since $t\isub{x}{u} =
        \app[\,]{s_1\isub{x}{u}}{s_2\isub{x}{u}}$ and $t'\isub{x}{u'}
        = \app[\,]{s'_1\isub{x}{u'}}{s'_2\isub{x}{u'}}$, one concludes
        this case as follows:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s_1\isub{x}{u}}
                    {s'_1\isub{x}{u'}}
                \hypoBangParF
                    {s_2\isub{x}{u}}
                    {s'_2\isub{x}{u'}}
                \inferBangParFApp
                    {\app[\,]{s_1\isub{x}{u}}{s_2\isub{x}{u}}}
                    {\app[\,]{s'_1\isub{x}{u'}}{s'_2\isub{x}{u'}}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangParFNameEsub$: Then there exist $s_1, s'_1,
        s_2, s'_2 \in \setBangTerms$ such that $t = s_1\esub{y}{s_2}$
        and $u = s'_1\esub{y}{s'_2}$ and so that the statement has the
        following form:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s_1}
                    {s'_1}
                \hypoBangParF
                    {s_2}
                    {s'_2}
                \inferBangParFEsub
                    {s_1\esub{y}{s_2}}
                    {s'_1\esub{y}{s'_2}}
            \end{prooftree}
        \end{equation*}
        By \ih (1) on $s_1 \bangParArrF s'_1$ and $s_2 \bangParArrF
        s'_2$, one obtains that $s_1\isub{x}{u} \bangParArrF
        s'_1\isub{x}{u'}$ and $s_2\isub{x}{u} \bangParArrF
        s'_2\isub{x}{u'}$. Since $t\isub{x}{u} =
        s_1\isub{x}{u}\esub{y}{s_2\isub{x}{u}}$ and $t'\isub{x}{u'} =
        s'_1\isub{x}{u'}\esub{y}{s'_2\isub{x}{u'}}$, one concludes
        this case as follows:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s_1\isub{x}{u}}
                    {s'_1\isub{x}{u'}}
                \hypoBangParF
                    {s_2\isub{x}{u}}
                    {s'_2\isub{x}{u'}}
                \inferBangParFEsub
                    {s_1\isub{x}{u}\esub{y}{s_2\isub{x}{u}}}
                    {s'_1\isub{x}{u'}\esub{y}{s'_2\isub{x}{u'}}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangParFNameDer$: Then there exist $s, s' \in
        \setBangTerms$ such that $t = \der{s}$ and $u = \der{s'}$ and
        so that the statement has the following form:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF{s}{s'}
                \inferBangParFDer
                    {\der{s}}
                    {\der{s'}}
            \end{prooftree}
        \end{equation*}
        By \ih (1) on $s \bangParArrF s'$, one obtains that
        $s\isub{x}{u} \bangParArrF s'\isub{x}{u'}$. Since
        $t\isub{x}{u} = \der{s\isub{x}{u}}$ and $t'\isub{x}{u'} =
        \der{s'\isub{x}{u'}}$, one concludes this case as follows:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s\isub{x}{u}}
                    {s'\isub{x}{u'}}
                \inferBangParFDer
                    {\der{s\isub{x}{u}}}
                    {\der{s'\isub{x}{u'}}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangParFNameOc$: Then there exist $s, s' \in
        \setBangTerms$ such that $t = \oc s$ and $u = \oc s'$ and so
        that the statement has the following form:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF{s}{s'}
                \inferBangParFOc{s}{s'}
            \end{prooftree}
        \end{equation*}
        By \ih (1) on $s \bangParArrF s'$, one obtains that
        $s\isub{x}{u} \bangParArrF s'\isub{x}{u'}$. Since
        $t\isub{x}{u} = \oc s\isub{x}{u}$ and $t'\isub{x}{u'} = \oc
        s'\isub{x}{u'}$, one concludes this case as follows:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s\isub{x}{u}}
                    {s'\isub{x}{u'}}
                \inferBangParFOc
                    {\oc s\isub{x}{u}}
                    {\oc s'\isub{x}{u'}}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangParFNameRefl$: Then $t = t'$ and we proceed by
        induction on $t$:
        \begin{itemize}
        \item[\bltII] $t = y$: We distinguish two cases:
            \begin{itemize}
            \item[\bltIII] $y = x$: Then $t\isub{x}{u} = u$ and
                $t'\isub{x}{u'} = u'$ which concludes this case since
                $u \bangParArrF u'$.

            \item[\bltIII] $y \neq x$: Then $t\isub{x}{u} = y$ and
                $t'\isub{x}{u'} = y$ and we concludes this case as
                follows:
                \begin{equation*}
                    \begin{prooftree}
                        \inferBangParFRefl
                            {y}
                            {y}
                    \end{prooftree}
                \end{equation*}
            \end{itemize}

        \item[\bltII] $t = \abs{y}{s}$: Then $t\isub{x}{u} =
            \abs{y}{s\isub{x}{u}}$ and $t'\isub{x}{u'} =
            \abs{y}{s\isub{x}{u'}}$. By \ih on $s$, one has that
            $s\isub{x}{u} \bangParArrF s\isub{x}{u'}$ and we concludes
            this case as follows:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s\isub{x}{u}}
                        {s\isub{x}{u'}}
                    \inferBangParFAbs
                        {\abs{y}{s\isub{x}{u}}}
                        {\abs{y}{s\isub{x}{u'}}}
                \end{prooftree}
            \end{equation*}

        \item[\bltII] $t = \app{s_1}{s_2}$: Then $t\isub{x}{u} =
            \app{s_1\isub{x}{u}}{s_2\isub{x}{u}}$ and $t'\isub{x}{u'}
            = \app{s_1\isub{x}{u'}}{s_2\isub{x}{u'}}$. By \ih on $s_1$
            and $s_2$, one has that $s_1\isub{x}{u} \bangParArrF
            s_1\isub{x}{u'}$ and $s_2\isub{x}{u} \bangParArrF
            s_2\isub{x}{u'}$. We then concludes this case as follows:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s_1\isub{x}{u}}
                        {s_1\isub{x}{u'}}
                    \hypoBangParF
                        {s_2\isub{x}{u}}
                        {s_2\isub{x}{u'}}
                    \inferBangParFApp
                        {\app{s_1\isub{x}{u}}{s_2\isub{x}{u}}}
                        {\app{s_1\isub{x}{u'}}{s_2\isub{x}{u'}}}
                \end{prooftree}
            \end{equation*}

        \item[\bltII] $t = s_1\esub{y}{s_2}$: Then $t\isub{x}{u} =
            s_1\isub{x}{u}\esub{y}{s_2\isub{x}{u}}$ and
            $t'\isub{x}{u'} =
            s_1\isub{x}{u'}\esub{y}{s_2\isub{x}{u'}}$. By \ih on $s_1$
            and $s_2$, one has that $s_1\isub{x}{u} \bangParArrF
            s_1\isub{x}{u'}$ and $s_2\isub{x}{u} \bangParArrF
            s_2\isub{x}{u'}$. We then concludes this case as follows:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s_1\isub{x}{u}}
                        {s_1\isub{x}{u'}}
                    \hypoBangParF
                        {s_2\isub{x}{u}}
                        {s_2\isub{x}{u'}}
                    \inferBangParFEsub
                        {s_1\isub{x}{u}\esub{y}{s_2\isub{x}{u}}}
                        {s_1\isub{x}{u'}\esub{y}{s_2\isub{x}{u'}}}
                \end{prooftree}
            \end{equation*}

        \item[\bltII] $t = \der{s'}$: Then $t\isub{x}{u} =
            \der{s\isub{x}{u}}$ and $t'\isub{x}{u'} =
            \der{s\isub{x}{u'}}$. By \ih on $s$, one has that
            $s\isub{x}{u} \bangParArrF s\isub{x}{u'}$ and we concludes
            this case as follows:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s\isub{x}{u}}
                        {s\isub{x}{u'}}
                    \inferBangParFDer
                        {\der{s\isub{x}{u}}}
                        {\der{s\isub{x}{u'}}}
                \end{prooftree}
            \end{equation*}

        \item[\bltII] $t = \oc s'$: Then $t\isub{x}{u} = \oc
            s\isub{x}{u}$ and $t'\isub{x}{u'} = \oc s\isub{x}{u'}$. By
            \ih on $s$, one has that $s\isub{x}{u} \bangParArrF
            s\isub{x}{u'}$ and we concludes this case as follows:
            \begin{equation*}
                \begin{prooftree}
                    \hypoBangParF
                        {s\isub{x}{u}}
                        {s\isub{x}{u'}}
                    \inferBangParFOc
                        {\oc s\isub{x}{u}}
                        {\oc s\isub{x}{u'}}
                \end{prooftree}
            \end{equation*}
        \end{itemize}
    \end{itemize}

\item $\bangLCtxt \bangParArrF \bangLCtxt'$: We distinguish two cases:
    \begin{itemize}
    \item[\bltI] $\bangParFNameHoleRefl$: Then $\bangLCtxt = \Hole$
        and $\bangLCtxt' = \Hole$ thus $\bangLCtxt\isub{x}{u} = \Hole$
        and $\bangLCtxt'\isub{x}{u'} = \Hole$ and one concludes this
        case as follows:
        \begin{equation*}
            \begin{prooftree}
                \inferBangParFHoleRefl
                    {\Hole}
                    {\Hole}
            \end{prooftree}
        \end{equation*}

    \item[\bltI] $\bangParFNameHoleEsub$: Then there exist terms $s,
        s' \in \setBangTerms$ and contexts $\bangLCtxt_1,
        \bangLCtxt'_1$ such that $\bangLCtxt =
        \bangLCtxt_1\esub{y}{s}$, $\bangLCtxt' =
        \bangLCtxt'_1\esub{y}{s'}$ and so that the statement has the
        following form:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {\bangLCtxt_1}
                    {\bangLCtxt'_1}
                \hypoBangParF
                    {s}
                    {s'}
                \inferBangParFHoleEsub
                    {\bangLCtxt_1\esub{y}{s}}
                    {\bangLCtxt'_1\esub{y}{s'}}
            \end{prooftree}
        \end{equation*}
        By \ih on $\bangLCtxt_1 \bangParArrF \bangLCtxt'_1$, one
        obtains that $\bangLCtxt_1\isub{x}{u} \bangParArrF
        \bangLCtxt'_1\isub{x}{u'}$. Similarly, by \ih on $s
        \bangParArrF s'$, one has that $s\isub{x}{u} \bangParArrF
        s'\isub{x}{u'}$. Since $\bangLCtxt\isub{x}{u} =
        \bangLCtxt\isub{x}{u}\esub{y}{s\isub{x}{u}}$ and
        $\bangLCtxt'\isub{x}{u'} =
        \bangLCtxt'\isub{x}{u'}\esub{y}{s'\isub{x}{u'}}$, one
        concludes this case as follows:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {\bangLCtxt_1\isub{x}{u}}
                    {\bangLCtxt'_1}
                \hypoBangParF
                    {s\isub{x}{u}}
                    {s'\isub{x}{u'}}
                \inferBangParFHoleEsub
                    {\bangLCtxt_1\isub{x}{u}\esub{y}{s\isub{x}{u}}}
                    {\bangLCtxt'_1\isub{x}{u'}\esub{y}{s'\isub{x}{u'}}}
            \end{prooftree}
        \end{equation*}
    \end{itemize}
\end{enumerate}
\end{proof}



\begin{lemma}
    The relation $\bangParArrF$ satisfies the diamong property.
\end{lemma}
\begin{proof}
Let $t, u_1, u_2 \in \setBangTerms$ such that $t \bangParArrF u_1$ and
$t \bangParArrF u_2$. We show that
$u_1 \bangParArrF t'$  and $u_2 \bangParArrF t'$.
We reason by induction on $t \bangParArrF u_1$:
\begin{itemize}
    \item[\bltI] $\bangParFNameBeta$: Then there exist terms $s_1,
    s_{1,1}, s_2, s_{1,2} \in \setBangTerms$ and context $\bangLCtxt,
    \bangLCtxt_1$ such that $t =
    \app{\bangLCtxt\bangCtxtPlug{\abs{y}{s_1}}}{s_2}$, $u_1 =
    \bangLCtxt_1\bangCtxtPlug{s_{1,1}\esub{x}{s_{1,2}}}$ and so that
    the statement has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypoBangParF
                {s_1}
                {s_{1,1}}
            \hypoBangParF
                {s_2}
                {s_{1,2}}
            \hypoBangParF
                {\bangLCtxt}
                {\bangLCtxt_1}
            \inferBangParFBeta
                {\app{\bangLCtxt\bangCtxtPlug{\abs{y}{s_1}}}{s_2}}
                {{\bangLCtxt_1}\bangCtxtPlug{s_{1,1}\esub{y}{s_{1,2}}}}
        \end{prooftree}
    \end{equation*}
    Since $t \bangParArrF u_2$, we distinguish two cases:
    \begin{itemize}
    \item[\bltII] $u_2 =
        \bangLCtxt_2\bangCtxtPlug{s_{2,1}\esub{x}{s_{2,2}}}$ and the
        statement has the following form:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {s_1}
                    {s_{2,1}}
                \hypoBangParF
                    {s_2}
                    {s_{2,2}}
                \hypoBangParF
                    {\bangLCtxt}
                    {\bangLCtxt_2}
                \inferBangParFBeta
                    {\app{\bangLCtxt\bangCtxtPlug{\abs{y}{s_1}}}{s_2}}
                    {{\bangLCtxt_2}\bangCtxtPlug{s_{2,1}\esub{y}{s_{2,2}}}}
            \end{prooftree}
        \end{equation*}
        for some terms $s_{2,1}, s_{2,2} \in \setBangTerms$ and some
        context $\bangLCtxt_2$. By \ih on $s_1 \bangParArrF s_{1,1}$
        with $s_1 \bangParArrF s_{2,1}$, one obtains that there exist
        $s'_1$ such that $s_{1,1} \bangParArrF s'_1$ and $s_{2,1}
        \bangParArrF s'_1$. \delia{By \ih on $s_2 \bangParArrF s_{1,2}$
        with $s_1 \bangParArrF s_{2,1}$, one obtains that there exist
        $s'_2$ such that $s_{1,2} \bangParArrF s'_2$ and $s_{2,2}
        \bangParArrF s'_2$. By \ih on $\bangLCtxt \bangParArrF \bangLCtxt_1$
        with $\bangLCtxt \bangParArrF \bangLCtxt_2$, one obtains that there exist
        $\bangLCtxt'$ such that $\bangLCtxt_1 \bangParArrF \bangLCtxt'$ and $
        \bangLCtxt_2\bangParArrF \bangLCtxt'$.}
        \delia{Then we conclude with $t'=\bangLCtxt'\bangCtxtPlug{s'_{1}
            \esub{x}{s'_{2}}}$ since $u_1\bangParArrF t'$ and $u_2\bangParArrF t'$. }

    \item[\bltII] $u_2 =
        \app{\bangLCtxt_2\bangCtxtPlug{\abs{y}{s_{2,1}}}}{s_{2,2}}$
        and the statement has the following form:
        \begin{equation*}
            \begin{prooftree}
                \hypoBangParF
                    {\bangLCtxt\bangCtxtPlug{\abs{y}{s_1}}}
                    {s_{2,1}}
                \hypoBangParF
                    {s_2}
                    {s_{2,2}}
                \inferBangParFApp
                    {\app{\bangLCtxt\bangCtxtPlug{\abs{y}{s_1}}}{s_2}}
                    {\app{s_{2,1}}{s_{2,2}}}
            \end{prooftree}
        \end{equation*}
        for some terms $s_{2,1}, s_{2,2} \in \setBangTerms$ and some
        context $\bangLCtxt_2$.
    \end{itemize}

    % By \ih on $\bangLCtxt \bangParArrF \bangLCtxt'$, one has that
    % $\bangLCtxt\isub{x}{u} \bangParArrF \bangLCtxt'\isub{x}{u'}$.
    % Similarly, by \ih on $s_1 \bangParArrF s'_1$ and $s_2
    % \bangParArrF s'_2$, one obtains that $s_1\isub{x}{u}
    % \bangParArrF s'_1\isub{x}{u'}$ and $s_2\isub{x}{u}
    % \bangParArrF s'_2\isub{x}{u'}$. Since $t\isub{x}{u} =
    % \app{\bangLCtxt\isub{x}{u}\bangCtxtPlug{\abs{y}{s_1\isub{x}{u}}}}{s_2\isub{x}{u}}$
    % and $t'\isub{x}{u'} =
    % \bangLCtxt\isub{x}{u'}\bangCtxtPlug{s'_1\isub{x}{u'}\esub{y}{s'_2\isub{x}{u'}}}$,
    % one concludes this case as follows:
    % \begin{equation*}
    %     \begin{prooftree}
    %         \hypoBangParF
    %             {s_1\isub{x}{u}}
    %             {s'_1\isub{x}{u'}}
    %         \hypoBangParF
    %             {s_2\isub{x}{u}}
    %             {s'_2\isub{x}{u'}}
    %         \hypoBangParF
    %             {\bangLCtxt\isub{x}{u}}
    %             {\bangLCtxt'\isub{x}{u'}}
    %         \inferBangParFBeta
    %             {\app{\bangLCtxt\isub{x}{u}\bangCtxtPlug{\abs{y}{s_1\isub{x}{u}}}}{s_2\isub{x}{u}}}
    %             {\bangLCtxt\isub{x}{u'}\bangCtxtPlug{s'_1\isub{x}{u'}\esub{y}{s'_2\isub{x}{u'}}}}
    %     \end{prooftree}
    % \end{equation*}

\item[\bltI] $\bangParFNameSubs$: Then $t =
    s_1\esub{y}{\bangLCtxt\bangCtxtPlug{\oc s_2}}$, $t' =
    \bangLCtxt'\bangCtxtPlug{s'_1\isub{y}{s'_2}}$ and so that the
    statement has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypoBangParF
                {s_1}
                {s'_1}
            \hypoBangParF
                {s_2}
                {s'_2}
            \hypoBangParF
                {\bangLCtxt}
                {\bangLCtxt'}
            \inferBangParFSubs
                {s_1\esub{y}{\bangLCtxt\bangCtxtPlug{\oc s_2}}}
                {\bangLCtxt'\bangCtxtPlug{s'_1\isub{y}{s'_2}}}
        \end{prooftree}
    \end{equation*}
    % By \ih on $\bangLCtxt \bangParArrF \bangLCtxt'$, one has that
    % $\bangLCtxt\isub{x}{u} \bangParArrF \bangLCtxt'\isub{x}{u'}$.
    % Similarly, by \ih on $s_1 \bangParArrF s'_1$ and $s_2
    % \bangParArrF s'_2$, one obtains that $s_1\isub{x}{u}
    % \bangParArrF s'_1\isub{x}{u'}$ and $s_2\isub{x}{u}
    % \bangParArrF s'_2\isub{x}{u'}$. Since $t\isub{x}{u} =
    % s_1\isub{x}{u}\esub{y}{\bangLCtxt\isub{x}{u}\bangCtxtPlug{\oc
    % s_2\isub{x}{u}}}$ and $t'\isub{x}{u'} =
    % \bangLCtxt'\isub{x}{u'}\bangCtxtPlug{s'_1\isub{x}{u'}\isub{y}{s'_2\isub{x}{u'}}}$,
    % one concludes this case as follows:
    % \begin{equation*}
    %     \begin{prooftree}
    %         \hypoBangParF
    %             {s_1\isub{x}{u}}
    %             {s'_1\isub{x}{u'}}
    %         \hypoBangParF
    %             {s_2\isub{x}{u}}
    %             {s'_2\isub{x}{u'}}
    %         \hypoBangParF
    %             {\bangLCtxt\isub{x}{u}}
    %             {\bangLCtxt'\isub{x}{u'}}
    %         \inferBangParFSubs
    %             {s_1\isub{x}{u}\esub{y}{\bangLCtxt\isub{x}{u}\bangCtxtPlug{\oc s_2\isub{x}{u}}}}
    %             {\bangLCtxt'\isub{x}{u'}\bangCtxtPlug{s'_1\isub{x}{u'}\isub{y}{s'_2\isub{x}{u'}}}}
    %     \end{prooftree}
    % \end{equation*}

\item[\bltI] $\bangParFNameBang$: Then $t =
    \der{\bangLCtxt\bangCtxtPlug{\oc s}}$, $t' =
    \bangLCtxt'\bangCtxtPlug{s'}$ and so that the statement has the
    following form:
    \begin{equation*}
        \begin{prooftree}
            \hypoBangParF
                {s}
                {s'}
            \hypoBangParF
                {\bangLCtxt}
                {\bangLCtxt'}
            \inferBangParFBang
                {\der{\bangLCtxt\bangCtxtPlug{\oc s}}}
                {\bangLCtxt'\bangCtxtPlug{s'}}
        \end{prooftree}
    \end{equation*}
    % By \ih on $\bangLCtxt \bangParArrF \bangLCtxt'$, one has that
    % $\bangLCtxt\isub{x}{u} \bangParArrF \bangLCtxt'\isub{x}{u'}$.
    % Similarly, by \ih on $s \bangParArrF s'$ one obtains that
    % $s\isub{x}{u} \bangParArrF s'\isub{x}{u'}$. Since
    % $t\isub{x}{u} = \der{\bangLCtxt\isub{x}{u}\bangCtxtPlug{\oc
    % s\isub{x}{u}}}$ and $t'\isub{x}{u'} =
    % \bangLCtxt'\isub{x}{u'}\bangCtxtPlug{s'\isub{x}{u'}}$, one
    % concludes this case as follows:
    % \begin{equation*}
    %     \begin{prooftree}
    %         \hypoBangParF
    %             {s\isub{x}{u}}
    %             {s'\isub{x}{u'}}
    %         \hypoBangParF
    %             {\bangLCtxt\isub{x}{u}}
    %             {\bangLCtxt'\isub{x}{u'}}
    %         \inferBangParFBang
    %             {\der{\bangLCtxt\isub{x}{u}\bangCtxtPlug{\oc s\isub{x}{u}}}}
    %             {\bangLCtxt\isub{x}{u'}\bangCtxtPlug{s'\isub{x}{u'}}}
    %     \end{prooftree}
    % \end{equation*}

\item[\bltI] $\bangParFNameAbs$: Then there exist $s, s' \in
    \setBangTerms$ such that $t = \abs{y}{s}$ and $u =
    \abs{y}{s'}$ and so that the statement has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypoBangParF{s}{s'}
            \inferBangParFAbs
                {\abs{y}{s}}
                {\abs{y}{s'}}
        \end{prooftree}
    \end{equation*}
    % By \ih on $s \bangParArrF s'$, one obtains that $s\isub{x}{u}
    % \bangParArrF s'\isub{x}{u'}$. Since $t\isub{x}{u} =
    % \abs{y}{s\isub{x}{u}}$ and $t'\isub{x}{u'} =
    % \abs{y}{s'\isub{x}{u'}}$, one concludes this case as follows:
    % \begin{equation*}
    %     \begin{prooftree}
    %         \hypoBangParF
    %             {s\isub{x}{u}}
    %             {s'\isub{x}{u'}}
    %         \inferBangParFAbs
    %             {\abs{y}{s\isub{x}{u}}}
    %             {\abs{y}{s'\isub{x}{u'}}}
    %     \end{prooftree}
    % \end{equation*}

\item[\bltI] $\bangParFNameApp$: Then there exist $s_1, s'_1,
    s_2, s'_2 \in \setBangTerms$ such that $t = \app{s_1}{s_2}$
    and $u = \app{s'_1}{s'_2}$ and so that the statement has the
    following form:
    \begin{equation*}
        \begin{prooftree}
            \hypoBangParF
                {s_1}
                {s'_1}
            \hypoBangParF
                {s_2}
                {s'_2}
            \inferBangParFApp
                {\app{s_1}{s_2}}
                {\app{s'_1}{s'_2}}
        \end{prooftree}
    \end{equation*}
    % By \ih on $s_1 \bangParArrF s'_1$ and $s_2 \bangParArrF s'_2$,
    % one obtains that $s_1\isub{x}{u} \bangParArrF
    % s'_1\isub{x}{u'}$ and $s_2\isub{x}{u} \bangParArrF
    % s'_2\isub{x}{u'}$. Since $t\isub{x}{u} =
    % \app[\,]{s_1\isub{x}{u}}{s_2\isub{x}{u}}$ and $t'\isub{x}{u'}
    % = \app[\,]{s'_1\isub{x}{u'}}{s'_2\isub{x}{u'}}$, one concludes
    % this case as follows:
    % \begin{equation*}
    %     \begin{prooftree}
    %         \hypoBangParF
    %             {s_1\isub{x}{u}}
    %             {s'_1\isub{x}{u'}}
    %         \hypoBangParF
    %             {s_2\isub{x}{u}}
    %             {s'_2\isub{x}{u'}}
    %         \inferBangParFApp
    %             {\app[\,]{s_1\isub{x}{u}}{s_2\isub{x}{u}}}
    %             {\app[\,]{s'_1\isub{x}{u'}}{s'_2\isub{x}{u'}}}
    %     \end{prooftree}
    % \end{equation*}

\item[\bltI] $\bangParFNameEsub$: Then there exist $s_1, s'_1,
    s_2, s'_2 \in \setBangTerms$ such that $t = s_1\esub{y}{s_2}$
    and $u = s'_1\esub{y}{s'_2}$ and so that the statement has the
    following form:
    \begin{equation*}
        \begin{prooftree}
            \hypoBangParF
                {s_1}
                {s'_1}
            \hypoBangParF
                {s_2}
                {s'_2}
            \inferBangParFEsub
                {s_1\esub{y}{s_2}}
                {s'_1\esub{y}{s'_2}}
        \end{prooftree}
    \end{equation*}
    % By \ih on $s_1 \bangParArrF s'_1$ and $s_2 \bangParArrF s'_2$,
    % one obtains that $s_1\isub{x}{u} \bangParArrF
    % s'_1\isub{x}{u'}$ and $s_2\isub{x}{u} \bangParArrF
    % s'_2\isub{x}{u'}$. Since $t\isub{x}{u} =
    % s_1\isub{x}{u}\esub{y}{s_2\isub{x}{u}}$ and $t'\isub{x}{u'} =
    % s'_1\isub{x}{u'}\esub{y}{s'_2\isub{x}{u'}}$, one concludes
    % this case as follows:
    % \begin{equation*}
    %     \begin{prooftree}
    %         \hypoBangParF
    %             {s_1\isub{x}{u}}
    %             {s'_1\isub{x}{u'}}
    %         \hypoBangParF
    %             {s_2\isub{x}{u}}
    %             {s'_2\isub{x}{u'}}
    %         \inferBangParFEsub
    %             {s_1\isub{x}{u}\esub{y}{s_2\isub{x}{u}}}
    %             {s'_1\isub{x}{u'}\esub{y}{s'_2\isub{x}{u'}}}
    %     \end{prooftree}
    % \end{equation*}

\item[\bltI] $\bangParFNameDer$: Then there exist $s, s' \in
    \setBangTerms$ such that $t = \der{s}$ and $u = \der{s'}$ and
    so that the statement has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypoBangParF{s}{s'}
            \inferBangParFDer
                {\der{s}}
                {\der{s'}}
        \end{prooftree}
    \end{equation*}
    % By \ih on $s \bangParArrF s'$, one obtains that $s\isub{x}{u}
    % \bangParArrF s'\isub{x}{u'}$. Since $t\isub{x}{u} =
    % \der{s\isub{x}{u}}$ and $t'\isub{x}{u'} =
    % \der{s'\isub{x}{u'}}$, one concludes this case as follows:
    % \begin{equation*}
    %     \begin{prooftree}
    %         \hypoBangParF
    %             {s\isub{x}{u}}
    %             {s'\isub{x}{u'}}
    %         \inferBangParFDer
    %             {\der{s\isub{x}{u}}}
    %             {\der{s'\isub{x}{u'}}}
    %     \end{prooftree}
    % \end{equation*}

\item[\bltI] $\bangParFNameOc$: Then there exist $s, s' \in
    \setBangTerms$ such that $t = \oc s$ and $u = \oc s'$ and so
    that the statement has the following form:
    \begin{equation*}
        \begin{prooftree}
            \hypoBangParF{s}{s'}
            \inferBangParFOc{s}{s'}
        \end{prooftree}
    \end{equation*}
    % By \ih on $s \bangParArrF s'$, one obtains that $s\isub{x}{u}
    % \bangParArrF s'\isub{x}{u'}$. Since $t\isub{x}{u} = \oc
    % s\isub{x}{u}$ and $t'\isub{x}{u'} = \oc s'\isub{x}{u'}$, one
    % concludes this case as follows:
    % \begin{equation*}
    %     \begin{prooftree}
    %         \hypoBangParF
    %             {s\isub{x}{u}}
    %             {s'\isub{x}{u'}}
    %         \inferBangParFOc
    %             {\oc s\isub{x}{u}}
    %             {\oc s'\isub{x}{u'}}
    %     \end{prooftree}
    % \end{equation*}

\item[\bltI] $\bangParFNameRefl$:
\end{itemize}
\end{proof}



\RecBangConfluence*
\begin{proof} \label{prf:Bang_Confluence}%
    \delia{[D: Je n'ai pas lu cette preuve]}
\end{proof}

